Exploration of Fast-Slow Latent Recurrence for Train-Short, Test-Long Generalization

We study out of distribution generalization in streaming tasks where models are trained on short sequences but must operate over much longer, unknown horizons under bounded memory. Our focus is on a persistent fast slow recurrent formulation in which a latent state is maintained across observations rather than reset at each stream step. For each incoming observation, the model performs multiple weight-shared latent updates with a recurrent core and then carries the resulting state forward to the next observation. This allows the model to maintain and refine a compact stream-level state without reprocessing a growing context. We evaluate this formulation across symbolic sequence prediction, supervised navigation, and partially observable reinforcement learning tasks. Across these settings, persistent latent recurrence improves OOD generalization over recurrent, state-space, and Transformer baselines. Through recurrent-core ablations, we identify architectural ingredients that are consistently associated with strong OOD performance, including state-dependent transitions and feature-wise nonlinear mixing. Together, these results highlight the value of revisiting persistent recurrence as an architectural bias for more generalizable sequence prediction.

==> abstract_ver1.tex <==
We investigate a combination of two mechanisms for building models that infer task-relevant rules from short sequential data and generalize them to out-of-distribution streaming inputs of unknown horizon: 
(1) recurrent computation with inner-loop updates between consecutive observations, and 
(2) latent recurrent reasoning modules originally developed for static inputs. 
Rather than treating each stream prefix as a separate static input, the resulting architecture applies a latent reasoning loop to each observation, performs several inner-loop updates in latent space, and then propagates the resulting latent state to the next stream step without reset. 
Through comparative experiments against prior recurrent mechanisms, alternative inner-loop cores, and static latent recurrent reasoning baselines, we show that this combination learns task-relevant patterns that persist across streaming inputs. 
On the Dyck language task, a model trained on sequences of length at most 40 generalizes to sequences longer than $10^5$. 
We further evaluate the mechanism on reinforcement-learning and navigation tasks, demonstrating out-of-distribution generalization to environments of unseen size.



% We investigate a combination of two mechanisms for building models that infer task-relevant rules from short sequential data and generalize them to out-of-distribution streaming inputs of unknown horizon: 
% (1) recurrent computation with inner-loop updates between consecutive observations, and 
% (2) latent recurrent reasoning modules originally developed for static inputs. 
% Rather than treating each stream prefix as a separate static input, the resulting architecture applies a latent reasoning loop to each observation, performs several inner-loop updates in latent space, and then propagates the resulting latent state to the next stream step without reset. 
% Through comparative experiments against prior recurrent mechanisms, alternative inner-loop cores, and static latent recurrent reasoning baselines, we show that this combination learns task-relevant patterns that persist across streaming inputs. 
% On the Dyck language task, a model trained on sequences of length at most 40 generalizes to sequences longer than $10^5$. 
% We further evaluate the mechanism on reinforcement-learning and navigation tasks, demonstrating out-of-distribution generalization to environments of unseen size.


% We investigate a combination of two mechanisms for building models that infer task-relevant rules from short sequential data and generalize them to out-of-distribution streaming inputs of unknown horizon: 
% (1) recurrent computation with inner-loop updates between consecutive observations, and 
% (2) latent recurrent reasoning modules originally developed for static inputs. 
% Rather than treating each stream prefix as a separate static input, the resulting architecture applies a latent reasoning loop to each observation, performs several inner-loop updates in latent space, and then propagates the resulting latent state to the next stream step without reset. 
% Through comparative experiments against prior recurrent mechanisms, alternative inner-loop cores, and static latent recurrent reasoning baselines, we show that this combination learns task-relevant patterns that persist across streaming inputs. 
% On the Dyck language task, a model trained on sequences of length at most 40 generalizes to sequences longer than $10^5$. 
% We further evaluate the mechanism on reinforcement-learning and navigation tasks, demonstrating out-of-distribution generalization to environments of unseen size.

==> conclusion_ver1.tex <==
\section{Conclusion and limitations}


We studied a fast--slow recurrent formulation that combines persistent recurrence over a stream with latent recurrent reasoning inside each observation step. 
By performing multiple latent updates per observation and propagating the resulting state without reset, the model adapts latent reasoning modules \maso{originally designed for static inputs to streaming settings.}

Across Dyck prediction, local maze navigation, and \Minigrid, this combination improves OOD generalization from short or small training instances to much longer streams or larger environments. 
Ablations show that inner-loop computation, weight sharing, and recurrent-core design all matter, with attention-based cores performing particularly well. 
The learned latents also organize around task-relevant variables such as stack depth and navigation events.

The present study also has several limitations. 
First, our method trades parallelism for expressivity: because the latent core is iterated multiple times per observation, inference is slower than highly optimized recurrent or state-space baselines. 
Although the proposed model is parameter-efficient, its current implementation does not yet exploit specialized kernels or recursion-aware parallelization. 
Second, our empirical study focuses on tasks where successful generalization can plausibly be supported by compact stream-level structure. 
The method should not be interpreted as solving arbitrary unbounded computation or arbitrary long-context reasoning. 
Third, while the latent visualizations reveal interpretable organization, they remain primarily diagnostic; establishing a causal connection between the observed attractor-like structures and OOD generalization requires further intervention-based analysis. 
Finally, we fixed or controlled the number of inner-loop iterations in order to isolate the effect of the recurrent core. 
Combining the proposed formulation with adaptive halting mechanisms, and understanding how to allocate computation dynamically across stream steps, remains an important direction for future work.

% We proposed a recurrent model that integrates sequential observations into recurrent modeling. Across the tasks that require long horizon information of task-relevant information while tending to incoming observation of varying relevance, our approach consistently outperformed strong baselines, including an LSTM, Mamba-2, and Transformer-XL, and it demonstrated competitive generalization and decision-making in dynamic environments. 
% This suggests the coupling of fast recurrent latent dynamics with slowly evolving observation dynamics as a promising mechanism for sequential inference over long-horizon.

% \paragraph{Limitations and future work}
% Despite strong performance on controlled benchmarks, our study has several limitations. 
% First, experiments are limited to relatively small-scale synthetic and grid-based domains, and we have not yet validated the approach on larger real-world tasks such as language, video, or robotics. 
% Second, the proposed fast-slow architecture incurs computational overhead due to its double-loop structure, resulting in lower GPU efficiency and slower inference than standard baselines (Appendix, Figure~\ref{fig:forward-speed}); improving efficiency via recursion-friendly parallelization methods (e.g., \citep{danieli2025pararnn}) is an important future direction. 
% Finally, we do note that there is a sensitivity to the random initialization, as observed in Figure~\ref{fig:results-minigrid}. 
% This suggests gradient instability from repeated layer reuse, as observed in RNNs~\citep{pascanu2013difficulty}, and motivates further architectural and optimization improvements.


%
% Finally, we observe sensitivity to random initialization, particularly in the Dyck experiments, where different seeds can lead to large OOD performance variance, suggesting gradient instability from repeated layer reuse, as observed in RNNs~\citep{pascanu2013difficulty}, and motivating further architectural and optimization improvements.


% We proposed a recurrent model that integrates sequential observations into iterative reasoning, thus bringing test‑time scaling to sequential decision‑making. Across maze‑solving and MiniGrid tasks, our approach consistently outperformed strong baselines, including an LSTM, Mamba, and Transformer‑XL, and it demonstrated superior generalization and decision‑making in dynamic environments. This highlights the value of coupling fast recurrent reasoning with slowly evolving observation dynamics and the value of auxiliary memory as a general mechanism for reasoning over streams of observations. However, the scope of our experiments is limited to controlled benchmarks, and scaling our method to larger, real‑world environments is an important direction for future work. \rev{We also note that our inner loops incur additional computational overhead relative to the baselines (see Figure~\ref{fig:t-scaling} in the Appendix). 
% A promising future direction of study also includes the application of recursion‑friendly parallelization strategies (e.g., parallel reductions~\citep{danieli2025pararnn})}


==> experiment_ver1.tex <==
\section{Experiment descriptions}\label{sec:exp}


\begin{wrapfigure}[8]{r}{0.6\textwidth}
\vspace{-1.0in}
    \centering
    \begin{subfigure}[t]{0.28\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/maze/id-sample.png}
        \caption{In-distribution ($19\times 19$)}
        \label{fig:sample-id}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.28\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/maze/ood-sample.png}
        \caption{OOD ($39\times 39$)}
        \label{fig:sample-ood}
    \end{subfigure}
    \caption{\Localmaze examples. Models are trained on small mazes (a) and evaluated on larger mazes (b). The green cell denotes the start, the red cell denotes the goal, and the observation is always limited to a $7\times 7$ region centered on the current position.}
    \label{fig:maze-sample}
\end{wrapfigure}


\begin{figure}[t]
\begin{minipage}{\columnwidth}
    \vspace{-.5em}
    \begin{subfigure}{0.49\linewidth}
    \hspace{-7mm}\includegraphics[width=1.2\linewidth]{figures/dyck/example_id.pdf}
      \caption{ID (random pattern)}
      \label{fig:dyck-id}
    \end{subfigure}
    \begin{subfigure}{0.49\linewidth}
      \hspace{-7mm}\includegraphics[width=1.2\linewidth]{figures/dyck/example_ood.pdf}
      \caption{OOD (1-regular run)}
      \label{fig:dyck-ood}
    \end{subfigure}
\end{minipage}

\caption{
Dyck examples. 
(a) The target at position $s$ is the token that closes the most recent unclosed bracket in the prefix up to $s$. When the stack is empty, ``$*$'' is predicted. 
(b) In a $1$-regular run, the predictor is required to output the token that closes the first open bracket (e.g., ``$[$'') at every odd step, while remembering this unresolved bracket for as long as the sequence continues.}
\label{fig:dyckexample}
\end{figure}



\subsection{Tasks}
We conduct experiments to verify out-of-distribution (OOD) generalization 
across three settings: symbolic stream prediction on the Dyck language 
\citep{dyckpaper}, navigation of a maze under egocentric observation 
(local maze), and reinforcement learning on \Minigrid
\citep{10.5555/3666122.3669331}.

\paragraph{Dyck.} 
We use Dyck-$(k,m)$~\citep{hewitt2020rnns}, a formal language with $k$ 
bracket types and maximum nesting depth $m$, to test whether the model 
can learn the underlying stack rule from short sequences(length $40$) and apply it 
to streams of unknown length. We set $k=30$ and $m=5$. Given a 
streaming input of brackets, the model predicts at each step $s$ 
the token that closes the most recently opened unclosed bracket; when 
no bracket is open, the prediction is ``\verb|*|''. For example, on 
input ``\verb|({[]|'', the prediction at $s=4$ should be ``\verb|}|'' 
(see Figure~\ref{fig:dyckexample}). Solving this requires tracking all 
unclosed brackets, whose number at step $s$ corresponds to the current 
stack depth and may grow with the sequence; once the structural rule 
is captured, the task admits arbitrary horizons.
\footnote{\citet{hewitt2020rnns} originally formulated Dyck as standard next-token prediction, but the type of the next \emph{opening} bracket is not deterministic; we therefore restrict the predictor to output only closing brackets and texttt{*}.}


\paragraph{\Localmaze.} 
\Localmaze extends the navigation task of \citet{CTM} and tests whether
a continuous, geometric rule learned on small mazes transfers to random mazes 
of substantially larger, unknown size (OOD). 
The model receives a stream of 
egocentric $7\times 7$ observations $O_s$ from a navigator that explores 
the maze under the right-hand rule (the model does not control the 
navigator),and must output the shortest path from start to goal as 
a sequence of actions (\texttt{up, down, left, right, pause}); the 
stream length $S$ varies with maze geometry. 
This task is importantly different from the one in \citet{CTM} because navigator's position
cannot be directly inferred from the egocentric vision. 
Solving this requires 
the model to integrate task-relevant observations while discarding 
information from dead-end branches, and to iteratively consolidate 
its hypothesis about the shortest path as new observations arrive. 
Supervision is the true shortest path, given at the end of each 
episode in the same action format; accuracy is measured by exact 
match on the predicted action sequence after removing \texttt{pause} 
tokens from both prediction and ground truth.


\paragraph{\Minigrid.} 
We finally evaluate on partially observable reinforcement learning 
tasks from \Minigrid~\citep{10.5555/3666122.3669331} to test whether
compositional rules such as ``pick up key, open door, reach goal'' 
can be learned \emph{online} from sparse reward and applied to 
environments substantially larger than those seen in training (OOD) . 
We use three tasks (Figure~\ref{fig:minigrid-description}): 
\textbf{DoorKey} (pick up a key, open a door, reach the goal, in this 
order), \textbf{MultiRoom} (open a sequence of doors to reach the 
goal), and \textbf{LavaCrossing} (reach the goal while avoiding lava). 
At each step, the agent receives an egocentric $7\times 7$ observation 
with object, color, and door-state channels, and selects an action 
$a_s \in \{\texttt{left}, \texttt{right}, \texttt{forward}, \texttt{toggle}, 
\texttt{pickup}, \texttt{drop}, \texttt{done}\}$. Reward is given only 
at the end of a successful episode; unlike Dyck and Local Maze, no 
ground-truth action sequence is provided, so the model must itself 
identify which observations are worth consolidating into its evolving 
plan.



\subsection{Ablative axes}
We conduct a series of ablations to identify which components of \eqref{eq:FastSlow} contribute to OOD generalization on the streaming tasks.
We used \Localmaze for many of the ablative studies as it relates to implicit rules in the space that is more continuous.
\maso{We conducted all experiments while aligning the wall-clock time per each observation. }

\paragraph{The framework \eqref{eq:FastSlow} itself.}
To validate that latent reasoning with continual injection of the input stream is more effective than prior approaches, we compare against the looped transformer of \citet{blayney2026mechanistic}, which is designed for inference over a static input sequence, and against CTM \citet{CTM}, a framework that infers from time-integrated synchronization patterns among the latents.
For the symbolic task of Dyck we also compare against the LLM models fine-tuned for the task. 

\paragraph{Effect of looping per observation.}
We ablate the loop length $T$ to verify that more thinking per observation improves OOD performance. As the $T = 1$ end of this axis, we include the standard recurrent baselines that perform no loop per observation, namely LSTM~\citep{LSTM} and Mamba~\citep{gu2023mamba}.

\paragraph{Shared weights.}
We verify that the benefit of weight sharing persists under our latent recurrent reasoning scheme. We compare \eqref{eq:FastSlow} against a variant in which the $T$ iterations are replaced by a stack of $T$ transformer layers with unshared weights, applied once per observation.


\paragraph{Choice of the recurrent core \core.}
To test the hypothesis that the attention structure used in \citet{Akorn, Looped} is important for OOD generalization, we compare \eqref{eq:FastSlow} against variants in which \core is instantiated as a CNN~\citep{CNN}, an LSTM, a linear attention block, or a Mamba block; the last of these recovers \citet{schone2025implicit}. We further ablate internal components of \core, including normalization layers and augmentative modules such as memory.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




% \begin{itemize}
% % \item Descrpition of the environments;  localMaze, RL, Dyck, etc 
% \item Ablation: Resets (Appendix) 
% \item Hyperparam? : (Appendix) 
% \item Ablation: Loop Numbers
% \item Ablation: Core choices
% \begin{itemize}
% \item AttnCores 
% \item Weight Sharing Cores
% \item Nonlinearity 
% \item Normalization 
% \item Delta From AKOrN 
% \end{itemize}

% \end{itemize}




% \begin{figure}[b!]
%     \begin{minipage}[t]{\columnwidth}
%     \vspace{0pt}
%         \centering
%         % (a)
%         \begin{subtable}[t]{0.48\columnwidth}
%             \centering
%             \includegraphics[width=\columnwidth]{figures/maze/id-smaple.png}
%             \caption{In-distribution ($19\times 19$)}
%             \label{fig:sample-id}
%         \end{subtable}
%         \hfill
%         % (b)
%         \begin{subfigure}[t]{0.48\columnwidth}
%             \centering
%             \includegraphics[width=\columnwidth]{figures/maze/ood-sample.png}
%             \caption{OOD ($39\times 39$)}
%             \label{fig:sample-ood}
%         \end{subfigure}
    
%         \captionof{figure}{
%         \Localmaze examples. Models are trained on small mazes (a) and evaluated on larger mazes (b). The green cell denotes the start, the red cell denotes the goal, and the observation is always limited to a $7\times 7$ region centered on its current position.
%             %Examples of maze environments. (a) In-distribution maze ($19\times19$). (b) Out-of-distribution maze ($39\times39$).
%         }
%         \label{fig:maze-sample}
%     \end{minipage}
% \end{figure}

% \section{Experiments}\label{sec:exp}

% We conducted a series of experiments to assess our model’s ability to dynamically integrate sequential inputs into its recurrent process in support of correct inference.
% We selected tasks that fundamentally require the model to iteratively and selectively identify task-relevant information from an evolving input sequence, and to consolidate it by continuously integrating this information into the latent state.

% We first present results on \Localmaze and Dyck tasks, both of which provide supervision in the form of correct answers. In these settings, the model can retrospectively infer which parts of the input are irrelevant to the correct underlying structure of the data.
% We additionally consider more challenging reinforcement learning tasks on MiniGrid. In these online settings, the model cannot directly compute the correct regret or value signal from immediate rewards, and therefore must learn indirectly how to integrate episodic information as it explores the environment.

% \paragraph{Hyperparameter}
% For the maze and Dyck tasks, we first identified a common set of training hyperparameters—specifically the number of epochs, batch size, and learning rate—for which validation performance converged across all baselines. After fixing these shared settings, we further tuned model-specific hyperparameters (e.g., learning rate and hidden dimensionality) independently for each baseline in order to maximize validation performance.
% %
% For the MiniGrid experiments, we adopted the same hyperparameters for all baselines as in \citet{ivan2025benchnetrl}, while tuning the hyperparameters of our proposed method separately.
% Also see Appendix (Tables~\ref{tab:hparams-merged} and \ref{tab:model-hparams-maze-minigrid}).


% \begin{figure*}[t]
%     \centering
%     \begin{subfigure}[b]{0.49\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/maze/id-main.pdf}
%         \caption{ID mazes ($19\times19$)}
%         \label{fig:maze-id}
%     \end{subfigure}
%     \hfill
%     %\hspace{1em}
%     \begin{subfigure}[b]{0.49\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/maze/ood-main.pdf}
%         \caption{OOD mazes ($39\times39$)}
%         \label{fig:maze-ood}
%     \end{subfigure}
%     \caption{Accuracy comparison of our model(\method) with baselines on the maze task. 
%     Our model(\method) shows substantially better OOD generalization. 
%     % \kohei{\texttt{Ours(V)} uses no auxiliary memory, \texttt{Ours(I)} uses internal memory, \texttt{Ours(E)} uses external memory, and \texttt{Ours(IE)} uses both.}
%     }
%     \label{fig:results-maze}
% \end{figure*}

% \subsection{\Localmaze} \label{sec:maze}

% The goal of this task is to infer the shortest path from the start to the end, while receiving a stream of egocentric observations from a navigator exploring the maze.  
% In this task, the information corresponding to dead-end paths is naturally task-irrelevant.
% In order for the model to be able to generalize its inference capability to OOD mazes of large size, the model must learn to efficiently integrate the task-relevant information and iteratively consolidate its hypothesis about the shortest path.

% More specifically, the model in this task is given a sequence of local, cropped $7\times 7$ neighborhood images $O_s$ corresponding to the egocentric observations of a navigator agent that explores the maze following the right-hand rule (the model has no control over the navigator).
% The navigator streams egocentric observations until the goal is reached. 
% The decoded output of the model is a sequence of movements (\texttt{up, down, left, right, pause}) corresponding to the estimated shortest path. 
% Depending on the geometry of the maze, the length of the observation sequence $S$ naturally varies across samples. 
% As a supervisory signal to be compared against the decoded output, we provide the model, at the end of each episode, with the true shortest path for the maze, represented in the same format. 
% We evaluate accuracy using a binary exact-match criterion on the entire predicted action sequence, after removing all \texttt{pause} tokens from both the prediction and the ground-truth shortest path.





% \paragraph{Setup}
% The mazes are generated randomly. 
% During training, they are of size $19 \times 19$. 
% We evaluate the model’s generalization on out-of-distribution (OOD) mazes of size $39 \times 39$.
% Figure~\ref{fig:maze-sample} shows examples of mazes for both the in-distribution (ID) and OOD settings.
% In the OOD setting, the observation sequence length $S$ tends to be naturally larger.

% We evaluate seven models on the maze task: LSTM, Transformer (TF), Mamba-2~\citep{dao2024transformers}, looped TF~\citep{Looped}, S5~\citep{smith2022simplified}, CTM~\citep{CTM}, and our model. Our dataset contains 45,000 training and 5,000 validation examples, in which training mazes are generated so that shortest‑path lengths are uniformly distributed.
% %We assess performance in both ID and OOD scenarios.
% For the default setting, we set $T=5$.
% Hyperparameters are tuned on the ID validation set and used unchanged for OOD evaluation. See Appendix~\ref{app:maze-details} for details. We report the mean $\pm$ sd over three seeds.


% % \paragraph{Designing \texorpdfstring{$J_t(X(t), C(s(t)))$}{J_t(X(t), C(t))} with Internal Memory}

% % Let the fast-time index be $t=0,1,2,\dots$ and the slow observation index be $s(t)=\lfloor t/T\rfloor$.
% % At each fast step, update the inner-loop and the internal memory causally:
% % \begin{align}
% % s_t &= \psi\!\bigl(X_t,\,C(s(t))\bigr), \\
% % h_{t+1} &= \mathrm{GRU}\!\bigl(s_t,\,h_t\bigr),
% % \label{eq:int-mem}
% % \end{align}
% % where $\psi$ is any function of the inner-loop state $X_t$ and the observation $C(s(t))$.

% % Define the objective at fast time $t$ as a continuous mapping of the internal memory:
% % \begin{align}
% % J_t \;\equiv\; J\!\bigl(\,\cdot\,;\,h_t,\,C(s(t))\bigr) \;:=\; \Phi(h_t)\,,
% % \end{align}
% % and constrain $\Phi$ to be Lipschitz (e.g., via spectral normalization or $1{\times}1$ convolutions). Then, for some constant $L>0$,
% % \begin{align}
% % \bigl\|J_{t+1}-J_t\bigr\| \;\le\; L\,\bigl\|h_{t+1}-h_t\bigr\|\,,
% % \label{eq:Lipschitz}
% % \end{align}
% % so $J_t$ evolves smoothly over fast time.


% \begin{table}[t]
% \centering
% \small
% \caption{
% Results of the maze task, represented in the format of  Mean $\pm$ std over 3 seeds. Layer=1 results describe how our recurrent structure with weight sharing performs with respect to $T_{train}$, the number of inner loop iterations in training.  
% $\text{Layers} > 1$ represent the results of multi-layer networks without weight sharing. 
% % \rev{Maze task results. Rows with $\text{Layers}=1$ correspond to the recurrent structure with weight sharing, where $T$ denotes the number of inner-loop iterations. Rows with $\text{Layers} > 1$ represent standard feedforward networks without weight sharing ($T=1$). Mean $\pm$ std over 3 seeds.}
% }
% \label{tab:maze_T_and_sharing_merged}
% %\resizebox{0.6\columnwidth}{!}{%
% \begin{tabular}{cc r @{$\,\pm\,$} l}
% \toprule
% Layers & $T_{train}$ & \multicolumn{2}{c}{OOD Acc.} \\
% \midrule
% \multirow{6}{*}{1} & 1  & 0.306 & 0.135 \\
%                    & 2  & 0.431 & 0.186 \\
%                    & 4  & 0.595 & 0.036 \\
%                    & 5  & 0.612 & 0.019 \\
% %                   & 8  & \bfseries 0.673 & \bfseries 0.006 \\
%                    & 8  &  0.673 & 0.006 \\
%                    & 16 & 0.673 & 0.032 \\
% \midrule
% 5                  & \multirow{2}{*}{1}  & 0.509 & 0.098 \\
% 10                 &                     & 0.445 & 0.164 \\
% \bottomrule
% \end{tabular}%
% %}
% \end{table}

% \paragraph{Results}

% Our model significantly outperforms all baselines on the maze task. As shown in Figure \ref{fig:results-maze}, it achieves near-perfect accuracy on the $19\times19$ (ID) mazes and, crucially, demonstrates strong generalization to unseen $39\times39$ mazes with approximately $60\%$ accuracy. In contrast, the baseline models all fail to generalize.

% % \begin{figure*}[h]
% %     \centering
% %     \begin{subfigure}[b]{0.49\textwidth}
% %         \includegraphics[width=\textwidth]{figures/maze/id-main.png}
% %         \caption{ID mazes ($19\times19$)}
% %         \label{fig:maze-id}
% %     \end{subfigure}
% %     \hfill
% %     \begin{subfigure}[b]{0.49\textwidth}
% %         \includegraphics[width=\textwidth]{figures/maze/ood-main.png}
% %         \caption{OOD mazes ($39\times39$)}
% %         \label{fig:maze-ood}
% %     \end{subfigure}
% %     \caption{Performance comparison of our model with baselinse on the Maze task. %Comparison of our model with baselines on (a) in-distribution ($19\times19$ mazes) and (b) out-of-distribution ($39\times39$ mazes). 
% %     Our model demonstrates superior generalization capability in the OOD setting.}
% %     \label{fig:results-maze}
% % \end{figure*}


% % \begin{figure*}[t]
% %     \centering
% %     \begin{subfigure}[b]{\columnwidth}
% %         \includegraphics[width=\columnwidth]{figures/maze/id-main.pdf}
% %         \caption{ID mazes ($19\times19$)}
% %         \label{fig:maze-id}
% %     \end{subfigure}
% %     \hfill
% %     \begin{subfigure}[b]{\columnwidth}
% %         \includegraphics[width=\columnwidth]{figures/maze/ood-main.pdf}
% %         \caption{OOD mazes ($39\times39$)}
% %         \label{fig:maze-ood}
% %     \end{subfigure}
% %     \caption{Accuracy comparison of our model with baselines on the maze task. 
% %     Our model shows substantially better OOD generalization. 
% %     % \kohei{\texttt{Ours(V)} uses no auxiliary memory, \texttt{Ours(I)} uses internal memory, \texttt{Ours(E)} uses external memory, and \texttt{Ours(IE)} uses both.}
% %     }
% %     \label{fig:results-maze}
% % \end{figure*}



% \paragraph{Effect of fast-loop iterations}
% The number of fast inner-loop iterations ($T$) controls how many recurrent updates occur between successive observations (Eq.~\ref{eq:FastSlow}). 
% To investigate whether the model benefits from longer recurrence, we conducted experiments with varying values of $T$ while keeping all other components fixed. 
% As shown in Table~\ref{tab:maze_T_and_sharing_merged}, OOD accuracy improves monotonically as $T$ increases, with gains saturating beyond $T=8$. 

% \paragraph{Effect of weight sharing (recurrence) in the fast loop}
% Our fast module applies the same update rule repeatedly for $T$ inner steps, i.e., it is \emph{recurrent} or \emph{weight-shared} across fast iterations. 
% To investigate the importance of this recurrent structure, we replaced it with an \emph{unrolled} residual stack of $T$ distinct layers, while keeping the overall fast--slow interface unchanged. 
% The results (Table~\ref{tab:maze_T_and_sharing_merged})
% show that weight sharing is crucial for OOD generalization: with the same inner-loop budget ($T{=}5$), the non-recurrent 5-layer stack reduces OOD accuracy from approximately $0.6$ to approximately $0.5$. 
% Increasing depth without sharing does not recover this performance: a 10-layer unshared stack further degrades OOD accuracy to approximately $0.45$, even after adjusting the learning rate. 
% These results support our design choice of a recurrent fast module.
% Please also see \ref{app:ablation_recurrent}.

% %The full details are in the Appendix~\ref{app:ablation_recurrent}.





% % \begin{table}[t]
% % \centering
% % \small
% % \setlength{\tabcolsep}{6pt}
% % \begin{tabular}{c c}
% % \toprule
% % Training-time $T$ & OOD Acc.\\
% % \midrule
% % 1  & $0.306 \pm 0.135$ \\
% % 2  & $0.431 \pm 0.186$ \\
% % 4  & $0.595 \pm 0.036$ \\
% % 8  & $\mathbf{0.673 \pm 0.006}$ \\
% % 16 & $0.673 \pm 0.032$ \\
% % \bottomrule
% % \end{tabular}
% % \caption{OOD accuracy on the maze task, varying fast inner-loop iterations $T$ used during training (mean $\pm$ std over 3 seeds). Increasing $T$ monotonically improves OOD generalization.}
% % \label{tab:T_train_scaling}
% % \end{table}

% % \begin{table}[t]
% % \centering
% % \small
% % \caption{OOD accuracy on the maze task, varying fast inner-loop iterations $T$ used during training (mean $\pm$ std over 3 seeds). Increasing $T$ monotonically improves OOD generalization.}
% % \label{tab:T_train_scaling}
% % \begin{tabularx}{\linewidth}{c Y}
% % \toprule
% % Training-time $T$ & OOD Acc.\\
% % \midrule
% % 1  & $0.306 \pm 0.135$ \\
% % 2  & $0.431 \pm 0.186$ \\
% % 4  & $0.595 \pm 0.036$ \\
% % 8  & $\mathbf{0.673 \pm 0.006}$ \\
% % 16 & $0.673 \pm 0.032$ \\
% % \bottomrule
% % \end{tabularx}
% % \end{table}


% % \subsection{Dyck-$(k,m)$}\label{sec:dyck}

% % \begin{figure}[t]
% % \vspace{-8pt}
% % \begin{subfigure}{1\textwidth}
% %   \centering  \includegraphics{figures/dyck/example_id.pdf}
% %   \vspace{-5pt}
% %   \caption{ID (random pattern)}
% %   \vspace{5pt}
% % \end{subfigure}
% % %-----------------(b)-----------------%
% % \begin{subfigure}{1\textwidth}
% %   \centering
% %   \includegraphics{figures/dyck/example_ood.pdf}
% %   \vspace{-5pt}
% %   \caption{OOD (1-regular run)}
% %   \vspace{5pt}
% % \end{subfigure}
% % \caption{Dyck language examples. 
% % %\rev{In 1-regular runs, the first open brackets (highlighted in red) reappear as prediction targets arbitrarily far into the sequence, testing the ability to retain information.}
% % (a) When the stack is empty, ``$*$'' is the next predicted token. 
% % (b) The predictor must remember ``['' forever while ``()'' continues in the input.}
% % \label{fig:dyckexample}
% % \end{figure}

% \begin{figure}[t]
% \begin{minipage}{\columnwidth}
%     \vspace{-.5em}
%     \begin{subfigure}{0.49\linewidth}
%     \hspace{-7mm}\includegraphics[width=1.2\linewidth]{figures/dyck/example_id.pdf}
%       \caption{ID (random pattern)}
%       \label{fig:dyck-id}
%     \end{subfigure}
%     \begin{subfigure}{0.49\linewidth}
%       \hspace{-7mm}\includegraphics[width=1.2\linewidth]{figures/dyck/example_ood.pdf}
%       \caption{OOD (1-regular run)}
%       \label{fig:dyck-ood}
%     \end{subfigure}
% \end{minipage}

% \caption{
% Dyck examples. 
% (a) The target at position $s$ is the token that closes the most recent unclosed bracket in the prefix up to $s$. When the stack is empty, ``$*$'' is predicted. 
% (b) In a $1$-regular run, the predictor is required to output the token that closes the first open bracket (e.g., ``$[$'') at every odd step, while remembering this unresolved bracket for as long as the sequence continues.}
% % \rev{In 1-regular runs, the first open brackets (highlighted in red) reappear as prediction targets arbitrarily far into the sequence, testing the ability to retain information.}
% % (a) When the stack is empty, ``$*$'' is the next predicted token. 
% % (b) The predictor must remember ``['' forever while ``()'' continues in the input.}
% \label{fig:dyckexample}
% \end{figure}



% \subsection{Dyck-$(k, m)$} \label{sec:dyck}

% We also experimented with the symbolic generalization task on Dyck-$(k,m)$~\citep{hewitt2020rnns}, with $k$ bracket types and maximum depth $m$. 
% Dyck is a stack-related task that heavily requires long-range lookup as well as iterative consolidation of the current stack structure, and it is the task referred to in the introduction. 
% We set $m=5$ and $k=30$.

% Given a streaming input of brackets as ``[\{([(('',  the goal is to sequentially predict the next bracket token that closes the most recent \emph{unclosed} bracket.
% For example, when the input sequence up to $s=4$ is ``\verb|({[]|'', the prediction at $s=4$ should be ``\}''. 
% When there is no bracket to close, the prediction should be ``*''; also see Figure~\ref{fig:dyckexample}. 
% % See \ref{app:dyck-details} for more details.
% % \footnote{\citet{hewitt2020rnns} originally formulated this task as standard next-token prediction. 
% %  However, because there are multiple valid choices for the type of the next open bracket, the task is not deterministic when formulated as pure next-token prediction. 
% % To eliminate this source of indeterminacy in accuracy evaluation, we restrict the predictor to output only the closing bracket.}


% % Given a streaming input of brackets $\{O_r \mid r < s\}$ (e.g., a sequence such as ``[, \{''), the goal is to sequentially predict the next bracket token $\hat{O}_s$ that closes the most recent \emph{unclosed} bracket.
% % \footnote{\citet{hewitt2020rnns} originally formulated this task as standard next-token prediction. 
% % However, because there are multiple valid choices for the type of the next open bracket, the task is not deterministic when formulated as pure next-token prediction. 
% % To eliminate this source of indeterminacy in accuracy evaluation, we restrict the predictor to output only the closing bracket.}
% % For example, when the input sequence up to $s=5$ is ``\verb|({[]|'', the prediction $\hat{O}_5$  should be ``)''.  
% % When there is no bracket to close in the previous tokens, the prediction should be ``*''; see Figure~\ref{fig:dyckexample}.  
% % Predictions are made sequentially at every $s$. 
% % For instance, if the sequence of \textit{input tokens} $O_{< 5}$ up to $s=4$ is ``\verb|()[{|'', the output sequence of \textit{predicted tokens}  $\hat{O}_{<5}$ is ``\verb|)*]}|''.


% The streaming sequence of brackets is analogous to an ever-growing stack of jobs, where the depth at time $s$ corresponds to the number of remaining brackets to close. 
% By design, this task requires the model to remember all unclosed brackets for as long as the sequence continues. 
% For example, for sequences of the form ``\verb|[()()()()|$\cdots$'' in Figure~\ref{fig:dyckexample}, the model must remember the unclosed ``\verb|[|'' as long as the sequence continues. 
% See \ref{app:dyck-details} for more details.

% \begin{figure*}[t]
%   \centering
%   \begin{tabular}{cc}
%     \begin{minipage}[c]{0.38\textwidth}
%       \centering
%       \includegraphics[width=\linewidth]{figures/dyck/acc_id.pdf} \\
%       \includegraphics[width=\linewidth]{figures/dyck/acc_ood.pdf}
%     \end{minipage}
%     & 

%     \begin{minipage}[c]{0.56\textwidth}
%       \centering
%       \includegraphics[width=\linewidth]{figures/dyck/energy.pdf}
%     \end{minipage}
%   \end{tabular}
%     \caption{Dyck results. \textbf{Left:} Token-wise prediction accuracy of Dyck sequences, plotted against length on ID (top) and OOD (bottom).
%     The shaded range indicates the sequence lengths used in training.
%     The ID strings are randomly generated under the constraint of bracket-depth $\le5$. For the OOD setting, we use 1-regular runs (see Figure~\ref{fig:dyckexample}).  
%     \textbf{Right:} An energy trace (See \ref{sec:choice}) for the first and second layers during a $5$-regular run, aligned with the input sequence (shown at the top of the plot).  
%     The energy of the first‑layer spikes with the arrival of a new bracket-\emph{type}, and then settles to the level specific to it. 
%     The energy of the second‑layer is organized by bracket-\emph{depth}. 
%     The dashed lines indicate the token arrival times.
%     }
%     \label{fig:dyck-acc-energy}
% \end{figure*}


% \paragraph{Setup}

% For the ID dataset, we randomly generate Dyck-$(30,5)$ strings.
% For the OOD dataset, we define a sequence to be an \textit{$n$-regular run} if it has the following structure:  
% (i) it begins with a random sequence of \textit{open} brackets of random length, and  
% (ii) it is followed by an infinite repetition of depth-$n$ openings and depth-$n$ closings.  
% For example, ``\verb|({[([[]](()){{}}|\dots'' is a $2$-regular run, and the one in Figure~\ref{fig:dyckexample} is a $1$-regular run.
% We use $1$-regular run for the OOD evaluation.
% % In general, $1$-regular runs is most difficult because predictions requiring memory of the initial ``\verb|[|'' constitute a higher proportion of the sequence (approximately $1/2$).

% We trained the model on 10{,}000 random strings in an ID dataset of length $\le 40$.  
% For evaluation, the model sequentially predicts on 1{,}000 $n$-regular runs of length up to 2{,}560.  
% Accuracy is computed for the prediction of each bracket.
% %
% We compare our model against LSTM, Transformer, and Mamba-2, which achieved relatively good performance in the maze experiments. 

% Since this task involves a hierarchical structure, we evaluate an extended variant of Eq.~\ref{eq:FastSlow} with two fast processes. 
% Specifically, for $\ell = 0,1,2$, we set $\bX^{(0)}(t) = \bC(t)$ and
% \begin{align*}\small
% \bX^{(\ell)}(t+1) = \Pi\left(\bX^{(\ell)}(t) + \gamma F\!\left(\bX^{(\ell)}(t), \bX^{(\ell-1)}(t)\right)\right)
% \end{align*}
% Predictions are obtained by decoding the last layer's output at each slow-time index $s$.  
% See Appendix~\ref{app:dyck-details} for details.



% \paragraph{Results}

% Figure~\ref{fig:dyck-acc-energy} shows token-level accuracy against the sequence length for both ID and OOD settings. 
% On ID data, all models except the vanilla Transformer extrapolate reasonably well across sequence lengths. 
% In contrast, on the OOD patterns of $1$-regular runs, all baselines eventually fall to the chance level ($0.5$) as the sequence length increases.
% This chance-level behavior corresponds to the cases of failing to predict the token that closes the first open bracket (colored red in Figure~\ref{fig:dyckexample}).
% Our model, however, maintains near $100\%$ accuracy over indefinitely long sequences, indicating that it retains the information of the first opening token while correctly predicting all other subsequent closures. 



% \paragraph{Comparison to LLMs}

% To relate this benchmark to current foundation models, we also compared our model against three frontier LLMs on the same Dyck-$(30,5)$ task (see Figure~\ref{fig:dyck-llms} in the introduction). 
% For the evaluation of our method in this comparative study, we used the model trained with the seed that attained the highest OOD accuracy at length 2,560 in producing Figure \ref{fig:dyck-acc-energy}. 
% In contrast to our model, which is trained only on raw Dyck strings of length $\le 40$, the LLMs are provided with a natural-language prompt describing the ground-truth algorithm that generates the sequence and are instructed to iteratively execute it; see \ref{app:dyck-details} for more details of the setup. 
% Despite their advantage in parameter scale and access to the explicit algorithm, their token-wise accuracy deteriorates as sequence length increases, whereas our model maintains accuracy above $90\%$ on sequences that are two orders of magnitude longer.

% \paragraph{Emergent structure in layerwise energies and latents}

% Interestingly, through learning the prediction task, our model discovers latent reasoning that aligns with the structural organization of the Dyck language. 
% Recall that for the recurrence used in our experiments (Section~\ref{sec:choice}), there exists an energy-like scalar that reflects the organizational level of the state. 
% We show the evolution of this energy in Figure~\ref{fig:dyck-acc-energy}, and the evolution of the latent in Figure~\ref{fig:dyck-pca}.
% %The evolution of this energy is shown in Figure~\ref{fig:dyck-acc-energy}, and the corresponding latent trajectories are shown in Figure~\ref{fig:dyck-pca}.
% %
% The energy of $X^{(1)}$ spikes upon the arrival of a new token and then stabilizes at a level that depends on the bracket type and whether the current token is opening or closing. 
% In contrast, the energy of $X^{(2)}$ is largely insensitive to bracket identity and is instead organized by stack \emph{depth}.
% This qualitative shift in energy organization indicates that the second fast process abstracts away from token identity and operates at a higher structural level.
% %
% PCA projections of the latents for both $X^{(1)}$ and $X^{(2)}$ support this interpretation: the state trajectories form a crisp, spring-shaped manifold indexed by stack depth that remains coherent over long horizons. 
% This structured organization in the learned latent space is similar to the report in 
% \cite{ouro2025} that the looped model tends to produce interpretable reasoning traces.
% This behavior stands in stark contrast to Mamba (Figure~\ref{fig:dyck-pca-mamba}).


% % \begin{wrapfigure}{r}{0.45\textwidth} % r = right, l = left
% %   \centering
% %   \vspace{-10pt} % optional: tweak vertical position
% %   \includegraphics[width=\linewidth]{figures/dyck/llms.pdf}
% %   \caption{\rev{Comparison with LLMs on Dyck. The shaded area indicates the training lengths.}}
% %   \label{fig:dyck-llms}
% % \end{wrapfigure}
% % \begin{figure}[tb]
% %   \centering
% %   \includegraphics[width=0.9\linewidth]{figures/dyck/llms.pdf}
% %   \caption{\rev{Comparison with LLMs on Dyck. The shaded area indicates the training lengths.}}
% %   \label{fig:dyck-llms}
% % \end{figure}
% % %

% %, showing that our model executes the streaming algorithm more reliably beyond the fixed context window.
% %The Dyck comparison therefore probes a regime in which both paradigms in principle admit more computation per input; LLMs through longer reasoning traces up to the token limit, and our model through larger $T$, yet only the proposed fast–slow recurrent architecture behaves as a reliable streaming algorithm executor beyond the fixed context window. 




% % ========= New Figure 8: PCA triptych (layer1, layer2, Mamba) =========
% % \begin{figure*}[tb]
% %   \centering
% %   \begin{subfigure}[b]{0.32\textwidth}
% %     \includegraphics[width=\textwidth]{figures/dyck/pca_1st.pdf}
% %     \caption{Ours: 1st-layer states}
% %     \label{fig:dyck-pca-1st}
% %   \end{subfigure}\hfill
% %   \begin{subfigure}[b]{0.32\textwidth}
% %     \includegraphics[width=\textwidth]{figures/dyck/pca_2nd.pdf}
% %     \caption{Ours: 2nd-layer states}
% %     \label{fig:dyck-pca-2nd}
% %   \end{subfigure}\hfill
% %   \begin{subfigure}[b]{0.32\textwidth}
% %     \includegraphics[width=\textwidth]{figures/dyck/pca_mamba.pdf}
% %     \caption{Mamba: last-layer states}
% %     \label{fig:dyck-pca-mamba}
% %   \end{subfigure}

% %   \caption{\rev{Comparison of latent state trajectories on a $5$-regular run of length 2,560. (a) PCA of the first-layer latents at the last fast step shows a star-shaped structure whose endpoints correspond to different opening brackets (color indicates bracket type). (b) The second-layer latents remain organized by stack depth (color) and opening/closing state ($\circ$ for open, $\times$ for close), indicating coherent, length-general computation. (c) Mamba's state trajectories at the last layer form a diffuse, overlapping cloud with frequent crossings and weaker organization by stack depth.  Mamba generalizes weaker in OOD domain.}}
% %   \label{fig:dyck-pca}
% % \end{figure*}
% \begin{figure*}[tb]
%   \centering
% \begin{minipage}{0.85\textwidth}
% \centering
% \begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}ccc@{}}
% \begin{subfigure}[b]{0.32\linewidth}
%   \includegraphics[width=\linewidth]{figures/dyck/pca_1st.pdf}
%   \caption{Ours: 1st-layer states}
% \end{subfigure}
% &
% \begin{subfigure}[b]{0.32\linewidth}
%   \includegraphics[width=\linewidth]{figures/dyck/pca_2nd.pdf}
%   \caption{Ours: 2nd-layer states}
% \end{subfigure}
% &
% \begin{subfigure}[b]{0.32\linewidth}
%   \includegraphics[width=\linewidth]{figures/dyck/pca_mamba.pdf}
%   \caption{Mamba: last-layer states}
%   \label{fig:dyck-pca-mamba}
% \end{subfigure}
% \end{tabular*}
% \end{minipage}
%   \caption{Comparison of latent trajectories of a $5$-regular run of length 2,560, visualized via PCA; $\circ$ marker indicates an open bracket and $\times$ marker indicates a close bracket. 
%   (a) Trajectory of the first layer latents of our model(\method). The color of the node indicates the bracket type. 
%   (b) Trajectory of the second layer latents of our model(\method). They are organized by stack depth (color) and opening/closing state. 
%   (c) Mamba's state trajectories at its last layer. They form a diffuse, overlapping cloud with frequent crossings and weaker organization. 
%   % \rev{Comparison of latent state trajectories on a $5$-regular run of length 2,560. (a) PCA of the first-layer latents at the last fast step shows a star-shaped structure whose endpoints correspond to different opening brackets (color indicates bracket type). (b) The second-layer latents remain organized by stack depth (color) and opening/closing state ($\circ$ for open, $\times$ for close), indicating coherent, length-general computation. (c) Mamba's state trajectories at the last layer form a diffuse, overlapping cloud with frequent crossings and weaker organization by stack depth.  Mamba generalizes weaker in OOD domain.}
%   }
%   \label{fig:dyck-pca}
% \end{figure*}
% % =====================================================================






% % \begin{figure}[t]
% %     \centering
% %     \begin{subfigure}[b]{0.45\linewidth}
% %         \centering
% %         \includegraphics[width=\linewidth]{figures/dyck/acc_id.pdf}
% %         \caption{ID (Random)}
% %     \end{subfigure}
% %     \hfill
% %     \begin{subfigure}[b]{0.45\linewidth}
% %         \centering
% %         \includegraphics[width=\linewidth]{figures/dyck/acc_ood.pdf}
% %         \caption{OOD ($1$-regular runs)}
% %     \end{subfigure}
% %     \caption{\rev{Dyck token accuracy by length. (a) ID denotes Dyck strings randomly generated under the constraint of depth $\le5$. (b) OOD denotes $1$-regular runs-strings with a random prelude followed by a long repeating “1 open then 1 close” pattern. The vertical dashed line marks the maximum training length. Our model preserves strong stack-tracking performance even on long OOD sequences.}}
% %     \label{fig:dyck-accuracy}
% % \end{figure}

% % \begin{figure*}[tb]
% %     \centering
% %     \begin{subfigure}[b]{0.45\textwidth}
% %         \includegraphics[width=\textwidth]{figures/dyck/energy.pdf}
% %         \caption{Energy}
% %         \label{fig:dyck-energy}
% %     \end{subfigure}
% %     \hfill
% %     \begin{subfigure}[b]{0.26\textwidth}
% %         \includegraphics[width=\textwidth]{figures/dyck/pca_1st.pdf}
% %         \caption{Layer1 state transition}
% %         \label{fig:dyck-pca-1st}
% %     \end{subfigure}
% %     \hfill
% %     \begin{subfigure}[b]{0.26\textwidth}
% %         \includegraphics[width=\textwidth]{figures/dyck/pca_2nd.pdf}
% %         \caption{Layer2 state transition}
% %         \label{fig:dyck-pca-2nd}
% %     \end{subfigure}
% %     \caption{\rev{Comparison of Dyck dynamics on $5$-regular runs. (a) Energy traces for the ``layer1'' and ``layer2'' modules. (b) PCA of the layer1 latents at the last fast step shows a star structure where the end points correspond to the open brackets, where the color indicates the bracket type at that point. (c) PCA of the layer2 latents remains organized by stack depth (different colors for the bracket depth) and open/close state ($\circ$ for open, $\times$ for close), indicating coherent, length-general computation.}}
% %     \label{fig:results-dyck}
% % \end{figure*}

% \subsection{Reinforcement Learning}\label{sec:rl}


% % \small
% \begin{figure*}[!b]
%   \centering
%   % --- このfigure内だけ詰める ---
%   \captionsetup{font=footnotesize,skip=2pt} % 図キャプション上の空き
%   \captionsetup[sub]{font=footnotesize,skip=1pt} % subcaption上の空き
%   \setlength{\tabcolsep}{3pt} % 列間（左右の間）
%   \renewcommand{\arraystretch}{0} % 行のデフォ伸びを抑える

%   \begin{tabular}{@{}cc@{}}
%     \subcaptionbox{LavaCrossing\label{fig:lava}}{%
%       \includegraphics[width=.4\textwidth,trim=8 6 8 6,clip]{figures/rl/lava-retry-4env-bars.pdf}} &
%     \subcaptionbox{DoorKey\label{fig:doorkey}}{%
%       \includegraphics[width=.4\textwidth,trim=8 6 8 6,clip]{figures/rl/doorkey-retry-4env-bars.pdf}} \\
%     \subcaptionbox{MultiRoom\label{fig:multiroom}}{%
%       \includegraphics[width=.4\textwidth,trim=8 6 8 6,clip]{figures/rl/multiroom-retry-4env-bars.pdf}} &
%     \subcaptionbox{All tasks\label{fig:alltask}}{%
%       \includegraphics[width=.4\textwidth,trim=8 6 8 6,clip]{figures/rl/alltasks-ID_OOD-avg-bars.pdf}}
%   \end{tabular}
%   \vspace{2mm}
%   \caption{Success rates on MiniGrid tasks, averaged over 5 random seeds. Error bars denote the standard deviation across seeds. Our model(\method) consistently matches or outperforms strong sequence-model baselines and achieves superior average performance across all tasks.}
%   \label{fig:results-minigrid}
% \end{figure*}

% % \begin{figure*}[t]
% %     \centering
% %     \captionsetup[subfigure]{labelformat=empty}
% %     \captionsetup[subfigure]{labelsep=none}

% %     % 左ブロック（2枚をグループ化、合計0.48）
% %     \begin{subfigure}[b]{0.48\textwidth}
% %         \centering
% %         \begin{subfigure}[b]{0.49\linewidth}
% %             \includegraphics[width=\linewidth]{figures/rl/doorkey5x5.png}
% %             \caption{DoorKey-5x5~(ID)}
% %             \label{fig:doorkey5x5}
% %         \end{subfigure}\hfill
% %         \begin{subfigure}[b]{0.49\linewidth}
% %             \includegraphics[width=\linewidth]{figures/rl/doorkey16x16.png}
% %             \caption{DoorKey\nobreakdash-16x16~(OOD)}
% %             \label{fig:doorkey_ood}
% %         \end{subfigure}
% %         % \caption{DoorKey environments} % グループにだけキャプション付けたい場合
% %     \end{subfigure}\hfill%
% %     % 右ブロック（各0.24）
% %     \begin{minipage}[b]{0.01\textwidth}
% %       \centering
% %       \begin{tikzpicture}
% %         \draw[dashed] (0,-2.0) -- (0,2.0);
% %       \end{tikzpicture}
% %     \end{minipage}\hfill%
% %     \begin{subfigure}[b]{0.24\textwidth}
% %       \includegraphics[width=\linewidth]{figures/rl/multiroomN6.png}
% %       \caption{MultiRoom(OOD)}
% %     \end{subfigure}\hfill%
% %     \begin{subfigure}[b]{0.24\textwidth}
% %       \includegraphics[width=\linewidth]{figures/rl/lavacrossingS11N5.png}
% %       \caption{LavaCrossing(OOD)}
% %     \end{subfigure}
% %     \caption{MiniGrid tasks. 
% %     The two left panels show the increasing difficulty from ID to OOD in DoorKey. MultiRoom and LavaCrossing likewise require long-horizon memory and reasoning.}
% %     \label{fig:minigrid-description}
% % \end{figure*}



% % \begin{figure*}[h]
% %     \centering
% %     \captionsetup[subfigure]{labelformat=empty}
% %     \captionsetup[subfigure]{labelsep=none}
% %     \begin{subfigure}[b]{0.24\textwidth}
% %         \includegraphics[width=\textwidth]{figures/rl/doorkey5x5.png}
% %         \caption{DoorKey-5x5~(ID)}
% %         \label{fig:doorkey5x5}
% %     \end{subfigure}
% %     \begin{subfigure}[b]{0.24\textwidth}
% %         \includegraphics[width=\textwidth]{figures/rl/doorkey6x6.png}
% %         \caption{DoorKey-6x6~(OOD)}
% %         \label{fig:doorkey}
% %     \end{subfigure}
% %     \begin{subfigure}[b]{0.24\textwidth}
% %         \includegraphics[width=\textwidth]{figures/rl/doorkey8x8.png}
% %         \caption{DoorKey-8x8~(OOD)}
% %         \label{fig:multiroom}
% %     \end{subfigure}
% %     \begin{subfigure}[b]{0.24\textwidth}
% %         \includegraphics[width=\textwidth]{figures/rl/doorkey16x16.png}
% %         \caption{DoorKey\nobreakdash-16x16~(OOD)}
% %         \label{fig:alltask}
% %     \end{subfigure}
% %     \caption{Examples of the partially observable MiniGrid environments used in our experiments. 
% %     These tasks, such as DoorKey of increasing sizes, require long-horizon memory and reasoning to solve. 
% %     Here,~\mbox{(ID)} denotes in-distribution and~\mbox{(OOD)} denotes out-of-distribution.} 
% %     \label{fig:minigrid-description}
% % \end{figure*}



% % \begin{figure}[t]
% %     \centering
% %     \begin{minipage}{0.52\linewidth}
% %         \centering
% %         \includegraphics[width=\linewidth]{figures/rl/energy_doorkey.pdf}
% %         \caption{\rev{Energy landscape in DoorKey. The red crosses indicate that the agent is adjacent to a wall at that step.}}
% %         \label{fig:doorkey_energy}
% %     \end{minipage}
% %     \hfill
% %     \begin{minipage}{0.45\linewidth}
% %         \centering
% %         \includegraphics[width=\linewidth]{figures/rl/visualize_doorkey.png}
% %         \caption{\rev{Latent state transitions of our model in DoorKey -$16 \times 16$(OOD) }}
% %         \label{fig:doorkey_pca}
% %     \end{minipage}
% % \end{figure}
% % \begin{figure}[t]
% %     \centering
% %     \begin{minipage}{0.52\linewidth}
% %         \centering
% %         \includegraphics[width=\linewidth]{figures/rl/energy_doorkey.pdf}
% %         \subcaption{\rev{Energy traces  (Eq.\ref{eq:Kenergy})  of the trajectories along a given episode. The red cross marks the timings at which the agent's relative view changes beyond a certain threshold. }}
% %         \label{fig:doorkey_energy}
% %     \end{minipage}
% %     \hfill
% %     \begin{minipage}{0.45\linewidth}
% %         \centering
% %         \includegraphics[width=\linewidth]{figures/rl/visualize_doorkey.png}
% %         \subcaption{\rev{Latent state trajectories of 30 episodes, visualized by PCA.}}
% %         \label{fig:doorkey_pca}
% %     \end{minipage}
% %     \caption{\rev{Energy and latent state trajectories in the DoorKey-16x16 (OOD) environment.}}
% %     \label{fig:doorkey_overall}
% % \end{figure}

% % \begin{figure}[t]
% %     \centering
% %     % [t] オプションで画像の上端を揃える
% %     \begin{minipage}[t]{0.52\linewidth}
% %         \centering
% %         \includegraphics[width=\linewidth]{figures/rl/energy_doorkey.pdf}
% %         \subcaption{\rev{Energy traces (Eq.\ref{eq:Kenergy}) along an episode. The red cross marks agent view changes.}}
% %         \label{fig:doorkey_energy}
% %     \end{minipage}
% %     \hfill
% %     \begin{minipage}[t]{0.45\linewidth}
% %         \centering
% %         \includegraphics[width=\linewidth]{figures/rl/visualize_doorkey.png}
% %         \subcaption{\rev{Latent state trajectories of 30 episodes, visualized by PCA.}}
% %         \label{fig:doorkey_pca}
% %     \end{minipage}
% %     \caption{\rev{Energy and latent state trajectories in the DoorKey-16x16 (OOD) environment.}}
% %     \label{fig:doorkey_overall}
% % \end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.85\linewidth]{figures/rl/energy_doorkey.pdf}
%     \caption{
%      Energy traces (See \ref{sec:choice}) along an episode in the DoorKey-16x16 (OOD) environment. \textbf{Top:} Event history along the trajectory. See the legend of Figure~\ref{fig:doorkey_pca} for event markings.  The red cross marks the changes in agent's view. \textbf{Bottom:} Energy trajectories.  }
%     \label{fig:doorkey_energy}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.75\linewidth]{figures/rl/visualize_doorkey.png}
%     \caption{
%     Latent state trajectories of 30 episodes for DoorKey-16x16 (OOD) environment, visualized by PCA.
%     Observe that important events are forming trajectory-independent clusters.}
%     \label{fig:doorkey_pca}
% \end{figure}

% We next evaluate our model on challenging partially observable reinforcement learning tasks from the MiniGrid environment \citep{10.5555/3666122.3669331}.
% We consider three MiniGrid tasks: DoorKey, MultiRoom, and LavaCrossing (see Figure~\ref{fig:minigrid-description}). 
% In these navigation tasks, DoorKey requires the agent to pick up a key, open a door, and then reach the goal in this order. 
% MultiRoom requires the agent to open multiple doors sequentially to reach the goal. 
% LavaCrossing requires the agent to reach the goal while avoiding the lava. 
% In all tasks, the reward is provided only at the end of a successful episode (i.e., sparse rewards).  

% Most importantly, because these tasks do not provide a ground-truth supervisory sequence of actions, it is more difficult for the model to retrospectively infer which information in the episode is worth incorporating into its reasoning and consolidating into intermediate conclusions.  

% At each slow step, the agent receives an egocentric $7\times7$ observation with object/color/door-state channels.
% The agent then selects an action from the set $a_s \in \{\texttt{left}, \allowbreak \texttt{right}, \allowbreak \texttt{forward}, \allowbreak \texttt{toggle}, \allowbreak \texttt{pickup}, \allowbreak \texttt{drop}, \allowbreak \texttt{done}\}$.

% \paragraph{Setup}
% We designed our evaluation protocol to test the model’s generalization capabilities in a zero-shot transfer setting. 
% The agent is trained exclusively on the simplest ID configuration and is subsequently evaluated, without any further training, on more complex and previously unseen OOD environments, which are typically larger than the ID environments (see Table~\ref{tab:env-id-ood} in the Appendix for details). 
% We compare our model against a few competitive sequence-modeling baselines, including LSTM, Mamba-2, and Transformer-XL. 
% Results are averaged over five random seeds, and we report the mean and standard deviation.

% All models are trained end-to-end using Proximal Policy Optimization (PPO; \citet{schulman2017ppo}).  
% For our model, the agent’s encoder (sensory module) first processes the input observations through a series of convolutional layers, followed by our recurrent core (Eq.~\ref{eq:FastSlow}).
% Please see Appendix~\ref{app:rl-details} for more details.



% \paragraph{Results}
% Figure~\ref{fig:results-minigrid} shows the success rates across all MiniGrid tasks. Our model performs comparably to or better than the baselines across all tested environments. This suggests that the recurrent mechanism of \textit{thinking while listening} is effective in these complex sequential decision-making problems as well.
% Also, we again observe a clear emergent structure in the latent space of our learned model. 
% We find that fluctuations in the energy value reflect the agent's level of ``frustration'', for example, when the agent's vision changes beyond a certain threshold (Figure~\ref{fig:doorkey_energy}). 
% Figure~\ref{fig:doorkey_pca} shows PCA-projected latent state transitions for DoorKey; irrespective of the trajectories, the model organizes its representations around key-events such as the ``key pickup'', ``door opening'', and ``goal discovery.'' 


% % Figure~\ref{fig:training-curve-doorkey}



% % \textbf{Designing \texorpdfstring{$J_t(X(t), C(s(t)))$}{J_t(X(t), C(t))} with External Memory}

% % Let the fast-time index be $t=0,1,2,\dots$ and the slow index be $s(t)=\lfloor t/T\rfloor$.
% % Aggregate past information into an external memory $m_t$ and update it causally:
% % \begin{align}
% % r_t &= \rho\!\bigl(X_t,\,C(s(t))\bigr), \\
% % m_{t+1} &= F\!\bigl(m_t,\,r_t\bigr),
% % \end{align}
% % where $\rho$ reads out from the current inner-loop output, and $F$ is any causal RNN (e.g., LSTM/GRU).

% % To ensure temporal continuity, define the objective at fast time $t$ as a continuous mapping of $m_t$:
% % \begin{align}
% % J_t \;\equiv\; J\!\bigl(\,\cdot\,;\,m_t,\,C(s(t))\bigr) \;:=\; \Phi(m_t)\,,
% % \end{align}
% % and constrain $\Phi$ to be Lipschitz (e.g., via spectral normalization, $1{\times}1$ convolutions, or small-step updates). Then, for some constant $L>0$,
% % \begin{align}
% % \bigl\|J_{t+1}-J_t\bigr\| \;\le\; L\,\bigl\|m_{t+1}-m_t\bigr\|\,,
% % \end{align}
% % so $J_t$ varies smoothly over time. 
% % This external-memory formulation is especially effective when the slow interval is long, as $m_t$ preserves continuity across extended gaps in $s$.



% % \paragraph{Test Time Scaling}

% % Figure~\ref{fig:tts-rl} illustrates the impact of varying $s$ on the agent's success rate across the three MiniGrid tasks. For all tasks, performance monotonically improves as $s$ is increased. This demonstrates that our model can effectively leverage additional computational budget at test time to enhance its decision-making quality. This graceful scaling property is highly desirable, as it allows for a flexible trade-off between computational cost and performance, enabling the deployment of the same trained model in various scenarios with different resource constraints.

% % \paragraph{Scaling with respect to $s$}
% % One the desiderate of our model is to feature the ability to reasoning that scales with the observation time $s$.
% % We therefore measured the models' behavior when we allowed longer durations (larger values) of $s$. 
% % We observe that the accuracy of our method generally improves with increasing $s$ for all environments (Figure~\ref{fig:tts-rl}).
% % While it is true that, for these experiments the accuracy itself shall scale with longer lenght of the episode length, our method improves faster and saturates at higher accuracy level than the competitors.  
% % \maso{For the DoorKey environment, however, LSTM surpasses our method beyond certain episode length because ...?} 


% % We posit that this is because the task in the DoorKey environment is bottlenecked by simple key discovery: in this setting, increasing $s$ merely lengthens the agent's dwell time spent in near-random wandering, passively raising the probability of encountering the key. Conversely, success in LavaCrossing and MultiRoom is predicated on goal-directed long-range dependencies, a context where such random exploration is entirely ineffective. This explains the limited performance gains of the standard LSTM baseline in these environments. In sharp contrast, our method with auxiliary memory is specifically designed to leverage these extra inner-loop iterations, enabling it to coherently integrate past observations and systematically refine the action plan.

% % \begin{figure*}[h]
% %     \centering
% %     \begin{subfigure}[b]{0.32\textwidth}
% %         \includegraphics[width=\textwidth]{figures/rl/test_time_scaling_doorkey.png}
% %         \caption{DoorKey}
% %         %\label{fig:tts_doorkey}
% %     \end{subfigure}
% %     \hfill
% %     \begin{subfigure}[b]{0.32\textwidth}
% %         \includegraphics[width=\textwidth]{figures/rl/test_time_scaling_lava.png}
% %         \caption{LavaCrossing}
% %         %\label{fig:doorkey}
% %     \end{subfigure}
% %     \hfill
% %     \begin{subfigure}[b]{0.32\textwidth}
% %         \includegraphics[width=\textwidth]{figures/rl/test_time_scaling_multi_room.png}
% %         \caption{MultiRoom}
% %         %\label{fig:doorkey}
% %     \end{subfigure}
% %     \caption{Effect of test-time scaling on the MiniGrid tasks, plotted against $s$, the slow process time scale.  The success rate consistently improves as the number of reasoning iterations increases at test time, highlighting the model's ability to leverage additional inference loops.}
% %     \label{fig:tts-rl}
% % \end{figure*}


==> intro_ver1.tex <==
\section{Introduction}



%Version 1
Latent recurrent reasoning, which iterates a weight-shared block in latent space, has recently emerged as a way to build reasoning capabilities directly into model architectures. 
This mechanism, \textit{especially with recurrent blocks with attention},  has been shown to enable strong reasoning performance  \citep{Geiping2025LatentReasoning, HRM, TRM, ouro2025, mcleish2025retrofit}, to represent programs and universal computation \citep{giannou2023programmable, xu2025expressive}, and, most relevantly to the present work, to learn and execute iterative algorithms at test time, which has been reported in the form of in-context regression, gradient-descent-like updates, and other pattern-driven procedures on the task with \textit{static input}~\citep{yang2024looped,Akorn, saunshi2025latent, Looped}.


We posit that the ability to learn a reusable algorithmic rule has a natural home that has not yet been explored in depth: \textbf{OOD generalization for the tasks with evolving input streams}, in which the model must process an unbounded 
sequence of observations $O(1), O(2), \ldots$ rather than a single fixed input.
Our argument is structural; in order for a system to process an \textit{unbounded} observation stream with \textit{bounded} memory and fixed-size state, one has no choice but to extract a rule that governs the evolution of the stream, while efficiently sorting out the information necessary for the rule.
For example, if we are to solve the Dyck task\citep{sinha2025illusion, hewitt2020rnns} of indefinite length, the only solution is to learn from the sequence the rule of "stack" structure.
This inspiration motivates us to investigate looped latent reasoning applied to evolving input. 
More particularly, we investigate the following system of continual loop of the latent $z$ with the recurrent core block $F$:
\begin{equation}
\lat^{(\ell+1)}(s) = \core \left(\lat^{(\ell)}(s), \obs(s)\right), \qquad \ell = 0, \ldots, T-1, \label{eq:mechanism_level0}
\end{equation}
where we loop $\core$ for $T$ times for each $\lat(s)$ received at observation timing $s$ and carry the latent forward to the next observation ($\lat^{(0)}(s+1)=\lat^{(T)}(s)$). 
Unlike \citet{Looped, blayney2026mechanistic}, this is a mechanism under which the latent looping does not "halt", so that the rule will be learned across the sequential observation.



We studied this mechanism across many choices of the recurrent core $\core$, and verified that the family of attention-based cores adopted in the aforementioned latent reasoning methods is notably stronger in terms of \textbf{OOD} generalization than alternatives such as \citep{LSTM,gu2023mamba, blayney2026mechanistic} on sequential tasks whose solution requires learning a reusable rule and applying it at every step. 
This mechanism also outperformed the standard Looped Transformer baseline~\citep{blayney2026mechanistic} applied auto-regressively to the sequential input, suggesting that loop must be carried across sequence for the capturing of the rule that governs the sequence.
Examining the learned latents, we also find that they are highly structured, forming a low-dimensional manifold indexed by task-relevant discrete states( e.g. stack depth in Dyck, key/door/goal events in \Minigrid~\citep{10.5555/3666122.3669331}) that is reused across the stream.
Concretely, on Dyck (30,5) \citep{hewitt2020rnns}, a canonical state-tracking benchmark, our model trained on sequences of length $\leq 40$ maintains $\approx 90\%$ token accuracy up to length $10^5$, which is four order of magnitudes beyond training.
Our method also outperforms continual reasoning methods like CTM~\citep{CTM} and other baselines \citep{} on OOD generalization for Reinforcement Learning tasks \citep{10.5555/3666122.3669331} as well as a maze navigation task with limited vision, demonstrating the ability to learn within a small environment a set of rules that can be applied in larger environment.


==> intro_ver2.tex <==
\section{Introduction}


%version2 

Humans can often extrapolate symbolic streams generated by a fixed rule far beyond the lengths observed during learning, or solve navigation puzzles of previously unseen size, after seeing only small, bounded examples. 
How can we endow machines with this capability?
We posit that this is not merely a question of memory maintenance: 
a finite-size memory cannot indefinitely store or attend to the raw history of an unbounded stream. 
Instead, the model must learn, from short observations, a compact task-relevant rule of the stream, such as its generative rule in symbolic streams, or a chain of subtasks in a puzzle that exists irrespective of stream length or environment size.
Latent recurrent reasoning, which iterates a weight-shared block in 
latent space, has recently emerged as a way to build related capabilities 
directly into model architectures 
\citep{Geiping2025LatentReasoning, HRM, TRM, ouro2025, mcleish2025retrofit}.
This mechanism, \emph{especially with recurrent blocks based on attention}, 
has been shown to represent programs and universal computation 
\citep{giannou2023programmable, xu2025expressive} and, most relevantly
to the present work, to learn and execute iterative algorithms at test 
time in the form of in-context regression, gradient-descent-like updates, 
and other pattern-driven procedures 
\citep{yang2024looped, Akorn, saunshi2025latent}.
Yet the in-depth study of these methods has so far focused on 
\emph{static input}: the loop iterates over a fixed input, and a naive 
application to unbounded stream tasks of the kind described above 
would require an indefinitely growing context. \\

We hypothesize that, by allowing the latent loop to persist alongside 
the stream, we can extend the ability of latent reasoning to capture, 
from a short sequence, the rules governing the input stream. 
We therefore investigate the following system of continual looping of 
the latent $\lat$ with a recurrent core block $\core$:
\begin{equation}
\lat^{(\ell+1)}(s) = \core\left(\lat^{(\ell)}(s),\, \mathbf{Encoder}(\obs(s))\right), 
\qquad \ell = 0, \ldots, T-1, \label{eq:continual-loop} 
\end{equation}
where $s \in \{1, 2, \ldots\}$ indexes observations along the stream, 
$\core$ is applied $T$ times for each $\obs(s)$ received at step $s$, and the 
latent is carried forward without reset: $\lat^{(0)}(s+1) = \lat^{(T)}(s)$.
This describes a dynamical system on the latent variable that is not reset at every observation step, and it reduces to a nonlinear RNN when $T=1$. 
\\

\maso{Our contribution is not the introduction of recurrence per se, but the combination of \textit{attention-based} latent recurrent reasoning with the persistent streaming formulation in \eqref{eq:continual-loop}, which extends latent recurrent reasoning from \textit{static-input inference} to OOD generalization on sequential tasks requiring reusable rules.
Indeed, related ideas have appeared in broader forms: adaptive computation methods such as ACT~\citep{ACT} can in principle be applied to any recurrent systems to modulate the amount of computation, while \citet{schone2025implicit} explore analogous persistent updates with Mamba-style cores in pursuit of a balance between parallelism and representation power.
In contrast, we study how the choice of $\core$ in \eqref{eq:continual-loop} affects OOD generalization on streaming inputs.}
Empirically, we find that attention-based cores, as used in recent
latent reasoning methods, yield strong OOD generalization.
Under comparable parameter budgets, attention-based cores outperform variants of the same persistent-loop formulation using alternative recurrent cores such as LSTMs~\citep{LSTM} and Mamba~\citep{gu2023mamba}, as well as a Looped Transformer baseline~\citep{blayney2026mechanistic} that treats the stream prefix observed so far as a static input at each step.

Concretely, on Dyck$(30,5)$ \citep{hewitt2020rnns, merrill2024illusion},
a canonical state-tracking benchmark, our model trained on sequences of 
length $\leq 40$ maintains $\approx 90\%$ token accuracy up to length 
$10^5$, four orders of magnitude beyond training.
Our method further outperforms continual-reasoning baselines such as 
CTM~\citep{CTM} on a limited-vision maze navigation task,
showing that rules learned in small environments can transfer to 
larger ones.
Examining the learned latents, we further find that they are highly 
structured: they form a low-dimensional manifold indexed by task-relevant 
discrete states (e.g., stack depth in Dyck, key/door/goal events in 
\Minigrid~\citep{10.5555/3666122.3669331}), and the dynamics reuse
representations, in that states sharing the same task-relevant features cluster together in latent space.



% \maso{We study the mechanism in \eqref{eq:continual-loop} across several choices of the recurrent core $\core$ and empirically show that attention-based cores, as used in recent latent reasoning methods, yield strong OOD generalization on streaming inputs.}


% \maso{Our contribution is not the introduction of recurrence per se, but the combination of latent recurrent reasoning with a streaming formulation in which the latent loop is propagated as a compact state across observations. }
% \maso{Within this formulation, we isolate the role of the recurrent core and empirically show that attention-based cores can extend the benefits of latent recurrent reasoning to OOD generalization tasks requiring systematic inference from streams of observations.}
% We study the mechanism in \eqref{eq:continual-loop} across several choices of the recurrent core $\core$ and empirically show that attention-based cores, as used in recent latent reasoning methods, yield strong OOD generalization on sequential tasks requiring reusable rules.

%and the same manifold is reused across the stream.


% How can we solve sequential tasks on evolving input streams of 
% % \emph{unbounded} horizon?


% when memory is bounded and cannot indefinitely extend the context, 
% one has no choice but to learn a rule that governs the evolution of 
% the stream and apply it repeatedly as new observations arrive.
% To this end, we propose to exploit recent advances in latent recurrent 
% reasoning, which iterates a weight-shared block in latent space and 
% has emerged as a way to build rule-exploiting reasoning capabilities 
% directly into model architectures 
% \cite{Geiping2025LatentReasoning, HRM, TRM, ouro2025, mcleish2025retrofit}.


% Yet the in-depth study of these methods has so far been confined to 
% \emph{static input}: even under auto-regressive application, the latents 
% are reset at each observation and the loop does not persist across the 
% stream, whereas the very setting from which we wish to extract a 
% governing rule is the long observation stream itself. \\  
% Since the rule we wish to extract governs the evolution of the entire stream, learning it requires \textit{reasoning} over the stream in its entirety, without halting between observations.
% Unlike the standard Looped Transformer \cite{Looped} under which the latent loop halts and is reset between inputs, the loop persists in this mechanism, so that the rule is learned across the stream.



% This mechanism also outperformed the standard Looped Transformer baseline \cite{mechanistic} applied auto-regressively to the sequential input, suggesting that the loop must be carried across the axis of stream evolution to capture the rule governing the stream.


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> method.tex <==
% \section{Latent Recurrent Model}\label{sec:recurrence_structure}

%\input{method_ver_1}
% \input{method_ver_ffn}

==> method_ver1.tex <==
\section{Latent Recurrent Model}\label{sec:recurrence_structure}


%% PURPOSE : TO HIGHLIGHT THE DIFFERENCE BETWEEN OURS AND LRM
Given a static observation $\obs$ of fixed length, the Latent Recurrent Model (\LRM) \citep{EBT, Geiping2025LatentReasoning, Akorn, Looped, yang2024looped} first processes $\obs$ through a \textit{prelude} encoder.
Starting from an initial latent $\lat^{\rm init} \in \RR^{\numtoken \times \latd}$ of $\numtoken$ tokens in $\latd$ dimension, the model sets $\lat(0) = \lat^{\rm init}$ and iteratively updates the latent state by injecting the fixed encoded input at every step over $t = 0, 1, \ldots, T-1$:
\begin{align}
\lat(t+1) = \core \left(\lat(t), \bC\right) \label{eq:LRM}
\end{align}
where $\mathrm{Encoder}(\obs) = \bC$.
The recurrence of this produces $\lat(T)$, a latent conclusion of depth $T$, which is passed through a \textit{coda} decoder, $\mathrm{Decoder}(\lat(T))$, for inference.
\citet{Geiping2025LatentReasoning, blayney2026mechanistic} instantiate $\core$ with a Transformer block, for example,
\begin{align}
    \core_{TF}(\lat(t), \bC )  = n_4(\tilde{\lat} + MLP(n_3(\tilde{\lat}))  ~~~\textrm{where} ~~~  \tilde{\lat}  = n_2(\lat(t) +  \textrm{Attn}(n_1(h[\lat(t), \bC])))) \label{eq:LRM}
\end{align}
where $\textrm{Attn}$ is the notation for usual Attention of mechanism as used in \citep{blayney2026mechanistic, Geiping2025LatentReasoning}, and 
$h$ is an adapter that merges $\lat$ with the observation, and $n_k$s are layer norms of choice.
However, this mechanism was built for the inference of fixed $\obs$, while our target is the stream of observations.




\section{Fast--Slow Coupling of Latent Recurrence with the Observational Process}
\label{sec:fastslow}

Since the rule we wish to extract governs the evolution of the entire stream, the latent recurrence must be allowed to run across observations rather than reset between them.
The family of models we investigate in this study implements this by injecting observations into a recurrence that is never reset.
Given a stream $\obs_1, \obs_2, \ldots, \obs_s, \ldots$ and an initial latent $\lat^{\rm init}$, we set $\lat^{(0)}(1) = \lat^{\rm init}$ and evolve the latent jointly with the stream according to
\begin{equation}
\label{eq:FastSlow}
\left\{
\begin{aligned}
\bC(s) &= \mathrm{Encoder}(\obs_s), \\[4pt]
\lat^{(\ell+1)}(s) &= \core \left(\lat^{(\ell)}(s), \bC(s); \theta\right), & \ell &= 1, \ldots, T, \\[4pt]
\lat^{(0)}(s+1) &= \lat^{(T)}(s),
\end{aligned}
\right.  
\end{equation}
for observation indices $s \in \{1, 2, \ldots, \}$.
Here, $\ell$ is the inner latent-recurrence index and $s$ is the (slower) observation index: the latent $\lat$ evolves $T$ times per observation, so the observation clock $s$ progresses $T$ times more slowly than the latent clock.
Inference is made from the decoded latent at each $s$.
\maso{We would refer to this mechanism as \method(\Method) for short.}
We investigate this mechanism under various choices of the recurrent core $\core$.
Although ACT~\citep{ACT} can be applied to \eqref{eq:FastSlow} in general to make $T$ adaptive, we will focus our study with fixed $T$ to isolate the design choice of $\core$ as well as \eqref{eq:FastSlow} itself.
Also, this mechanism can be used in hierarhical form for better stability and stronger representation as well, please see \eqref{fig:code-meta}.


\subsection*{Recurrent core with Attention mechanism}

We will show that choices of $\core$ equipped with an attention mechanism are particularly successful at OOD generalization on sequential tasks that require learning a rule governing the stream.
In particular, as we elaborate in the experiments section, the family of cores of the $\core_{TF}$ yielding
\begin{align}
\lat^{(\ell+1)}(s) = \core_{TF} \left(\lat^{(\ell)}(s), \bC(s); \theta\right)
\end{align}
and its extensions such as the one used by \citet{Akorn} proved particularly strong.
achieving the best OOD performance.
One commonality shared across the family of $\core_{TF}$ and its extension we explored is their tendency to iteratively form stable and metastable configurations in the latent trajectory, a phenomenon which has been reported both empirically \citep{blayney2026mechanistic} and theoretically \citep{geshkovski2024dynamic, geshkovski2025mathematical, Kuramoto} in the static-input setting of \eqref{eq:LRM}.
We observe that the analogous phenomenon emerges in the latent trajectory of \eqref{eq:FastSlow} with $\core_{TF}$, and that the model captures the rule governing the stream through reusable representations associated with these (meta)stable configurations.
In the static-input setting, \citet{geshkovski2024dynamic} associates such stability with an energy of the form
\begin{equation}
E(\lat) = - \sum_{i,j \in 1:\numtoken} [\mathrm{AttnMat}_\theta(\lat)]_{ij} \lat_i^\top  \lat_j, \label{eq:energy}
\end{equation}
where $\lat_i$ denotes the $i$-th token of $\lat$ and $[\mathrm{AttnMat}_\theta(\lat)]_{ij}$ is the $(i,j)$-th entry of the token-coupling attention matrix; the AKOrN architecture \citep{Akorn} adopts a similar energy.
We will use this energy to visualize the relationship between the learned latent trajectory and the ground-truth rule governing the stream.




% When $\core$ is instantiated with a Transformer block, for example, one way to apply \eqref{eq:LRM} to a sequential task such as next-token or next-frame prediction is auto-regressive: at each observation index $s$, the model is run on the accumulated context $(\obs_1, \ldots, \obs_s)$ under the usual causal mask, with the latent recurrence re-initialized to $\lat^{\rm init}$ at the start of each step.
% A related strategy, pursued in the single-task reasoning setting by \citet{hao2024training}, is to additionally feed the latent produced at each step (or its decoded form) back as input to the model, so that the accumulated latents $\{\lat^{s}(T)\}_{s}$ form part of the context at subsequent steps.
% Both routes cause the context length to grow with $s$, and excessively long contexts are known to suffer from well-documented degradation \cite{liu2023lost, shojaee2025illusion2}, making neither strategy well suited to an unbounded stream of inputs.

% Our method is inspired by models that conduct reasoning in the latent space by iterating a recurrent block \cite{EBT,Geiping2025LatentReasoning,Akorn}.   
% Given a specified number of recurrent iterations $T$ at training time, this class of approaches takes an observation $O$ as input together with an initial noise tensor $\bX_0 \in \mathbb{R}^{K \times D}$, where $K$ is the number of latent tokens and $D$ is the model dimension.
% The model then iteratively updates the latent state $\bX(t)$ by initializing $\bX(0)=\bX_0$ and applying
% \begin{align}
% \bX(t+1) = R\left(\bX(t), \mathrm{Encoder}(O)\right)
% \end{align}
% for $t = 0,1,\dots,T-1 .$
% This produces $\bX(T)$, a latent conclusion of depth $T$. We use $\mathrm{Decoder}(\bX(T))$ for inference.  

% This system can be applied autoregressively; for example, one may set $\mathrm{Decoder}(\bX(T))$ to serve as the next observation $O$ in a subsequent round of reasoning. 
% When applied autoregressively at turn index $s$, models in this family typically use the accumulated set of the latent tokens $\bX^{s}(T)$, or its decoded form, as contextual input, and reinitialize $\bX^{s}(0)$ at every turn \cite{EBT,hao2024training}.
% %
% A naive extension of this strategy to an evolving observation sequence $O_s$ is to concatenate $\{\bX^{s}(T)\}_{s}$ with $\{O_s\}_{s}$ as context, which causes the context length to grow with increasing $s$. 
% This introduces one source of long-horizon failure, namely the difficulty associated with the use of excessively long contexts \cite{liu2023lost, shojaee2025illusion2}.
% In the next section, we extend the latent recurrent model more directly so that the reasoning proceeds continuously while \textit{listening} to an evolving stream of observations.


% This approach stands in contrast to models that scale computation by producing more tokens to condition.
% Without requiring supervisory signals for the reasoning process, these models are reported to capture types of reasoning that are not easily represented in words. 
%

% Our goal is to explore a system that can continuously integrate the evolving external signals into the latent reasoning process.
% To this end, we modify latent recurrent reasoning by considering a coupled dynamical system in which the observational process and the reasoning process evolve on the same timeline but at different speeds. 
% In our model, the reasoning process proceeds $T$ times faster than the observation process, so that $T$ also represents the number of latent reasoning iterations performed per observation.

% Let $t$ denote the fast time scale, and let $s=\lfloor t/T \rfloor$ denote the slow time scale indexing the observations, with observations given by $O_s$.
% Let $\bC(t)\in \mathbb{R}^{K \times D}$ denote the encoded observation process and $\bX(t)$ denote the latent process of thought, operating in the same latent space as $\bC(t)$. 
% The discretized dynamics of our model are given by
% \begin{equation}
% \label{eq:FastSlow}
% \left\{
% \begin{aligned}
% \bC(t) &= \mathrm{Encoder}(O_s) \\ 
%      & \hspace{0.5cm} \text{for } s = \lfloor t/T \rfloor \in \{0,\dots,S-1\}, \\[6pt]
% \bX(t+1) &= \Pi\left(\bX(t) + \gamma F\left(\bX(t), \bC(t); \theta\right)\right) \\
%        & \hspace{0.5cm} \text{for } t \in \{0,\dots,ST-1\},
% \end{aligned}
% \right.
% \end{equation}
% where $F$ is a neural network parameterized by $\theta$ and shared across timesteps, $\gamma>0$ is the step size, and $\Pi(\bx)=\bx/\|\bx\|$ is a normalization operator.
% When the observation sequence has length $S$, the recurrent module performs a total of $ST$ latent updates while receiving $S$ encoded observation signals. 
% Importantly, this differs from standard latent recurrent reasoning in that the time axis of the observation process is aligned with that of the fast latent reasoning, whose state transitions persist over time. 

% The latent state is initialized as $\bX(0)\sim\mathcal{N}(0,I)$ at the beginning of each episode and is \textbf{never reset} until the episode ends; instead, it continuously moves forward in time and integrates the slow evolution of $\bC(t)$ into its dynamics, even when the observational process evolves independently of $\bX(t)$.
% See Figure \ref{fig:fastslowTask} for visualization of our scheme.

% %
% We train the parameters $\theta$ and $\gamma$ as well as the encoder and decoder for various tasks that use the sequential output of $\bX(t)$ for inference. 
% For the prediction task on the observation sequence, $O_{s+1}$ is predicted by $\mathrm{Decoder}(\bX(sT))$.  

% \subsection{The Choice of $F$}\label{sec:choice}

% For the choice of $F$ in our experiment, we explored a mechanism related to the architecture with self-organization properties \cite{Kuramoto, geshkovski2025mathematical,geshkovski2024dynamic}.
% % For the choice of $F$ in our experiment, we explored a mechanism that has been reported to have self-organization and metastable property \cite{geshkovski2025mathematical,geshkovski2024dynamic, Kuramoto}.
% In particular, we used the approach of \citet{Akorn} with attention-type update as follows: 
% \begin{align}
% F(\bX, \bC)_i &:= \bOmega_i \bx_i+ \mathrm{Proj}_{\bx_i}\Big( J(\bX, \bC)_i \Big) \label{eq:kupdate}
% \end{align}
% where $\bx_i$ is the $i$-th latent token in $\bX$, $\mathrm{Proj}_{\bx}(\bv)=\bv - (\bv^\top \bx)\bx$ is the projection of the vector onto the tangent of the unit sphere, $\bOmega_i$ is an anti-symmetric matrix, and each $\bx_i(t)$ is normalized so that the latent tokens remain on the unit sphere for every $t$. 
% Following  \citet{Akorn}, our $J$ is an attention-based function that mixes latent tokens $\{\bx_i\}$ while integrating $\bC$ in an additive manner. 
% Please see Appendix~\ref{app:impl-J} for details. 
% We also observe that a variant where $J$ is implemented as a vanilla Transformer block works competitively as well, but the model based on \citet{Akorn} performed most stably (Appendix~\ref{app:fast-module}).

% \paragraph{Energy-like scalar}

% This model also provides a scalar quantity that is useful for tracing the behavior of the latent updates.
% The update can be interpreted as a dynamical system of interacting latent tokens evolving toward self-organization, and there exists a tractable, energy-like scalar that represents the degree of self-organization of the neuronal population \cite{Kuramoto}; see Appendix \ref{sec:energy}.
% In the experimental section, we will demonstrate that our model learns to dynamically align the interpretable structural properties of the system with this energy state.


==> results_ver1.tex <==
\section{Quantative Results}

\subsection{The effectiveness of \eqref{eq:FastSlow} itself with attention-based core} 


Across all settings (\Localmaze, Dyck, and \Minigrid), our model \eqref{eq:FastSlow} with an attention-based core performed competitively in the training regime and outperformed the baselines in the OOD regime, including LSTM~\citep{LSTM} and Mamba~\citep{gu2023mamba}.
For the explicit design of $R$ representing our approach, we used \citet{Akorn} and \citet{blayney2026mechanistic}, \maso{for which we provide more detailed descriptions in Appendix~\ref{app:impl-J}}.
For \Localmaze, see Figure~\ref{fig:results-maze}, where all baselines fail to generalize on the mazes of unseen size.
For Dyck (Figures~\ref{fig:dyck-llms} and \ref{fig:dyck-acc-energy}), note that the methods with $T=1$ fail early in the OOD range $10^3 <$, and the fine-tuned LLMs follow suit, though at a slower rate.
\kohei{The frontier LLM comparison in Figure~\ref{fig:dyck-llms} is a zero-shot API evaluation with algorithmic hints, which is asymmetric because \method is trained directly on Dyck. To reduce this asymmetry, we also fine-tuned the open-weight Qwen3-4B-Base model on the same Dyck-$(30,5)$ split and protocol. Qwen3-4B-Base reaches high accuracy at in-distribution lengths, but under the same $1$-regular OOD protocol its accuracy drops toward chance, reaching approximately $50\%$ at length $20{,}480$.}
Our method, on the other hand, generalizes to lengths beyond $10^5$ when trained on sequences of length $40$.
Our model also achieves better OOD performance than the baselines on the \Minigrid reinforcement-learning tasks(larger environment size).
We outperform TransformerXL~\citep{dai2019transformer} on this task as well.
Overall, we confirm that our model \eqref{eq:FastSlow} with an attention-based core is a promising approach for OOD tasks on unbounded streaming inputs, compared to both classical approaches designed for static inputs and RNN-like methods without an internal loop ($T=1$). 

\begin{figure*}[ht!]
    \centering
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/maze/id-main.pdf}
        \caption{ID mazes ($19\times19$)}
        \label{fig:maze-id}
    \end{subfigure}
    \hfill
    %\hspace{1em}
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/maze/ood-main.pdf}
        \caption{OOD mazes ($39\times39$)}
        \label{fig:maze-ood}
    \end{subfigure}
    \caption{Accuracy comparison of our model (\method) with baselines on the maze task. 
    Our model (\method) shows substantially better OOD generalization. 
    }
    \label{fig:results-maze}
\end{figure*}



\begin{figure}[ht!]
    \centering
      \includegraphics[width=0.9\linewidth]{figures/dyck/llms.pdf}
    \caption{Token-wise accuracy vs. sequence length on the Dyck-$(30,5)$ task. 
Frontier LLMs are prompted with the ground-truth generation algorithm of the Dyck language in text form, so that they only need to execute the plan described in the prompt; see Appendix~\ref{app:dyck-details} for the exact prompt and the evaluation protocol.
Their performance drops rapidly as sequence length increases, consistent with the behavior reported by \citet{shojaee2025illusion2,sinha2025illusion}. 
\kohei{Qwen3-4B-Base is included as an open-weight LoRA fine-tuned baseline trained on the same short Dyck split and evaluated on the same $1$-regular OOD protocol.}
%The maximum evaluated length is capped by API output limits; beyond this point we cannot measure accuracy for these models.
Our model (\method), in contrast, is trained exclusively on raw strings of short length (shaded range, $\leq 40$). 
It maintains approximately $90\%$ accuracy over sequence lengths spanning four orders of magnitude beyond the training range.}
    \label{fig:dyck-llms}
\end{figure}


\begin{figure*}[!bht]
  \centering
  % --- このfigure内だけ詰める ---
  \captionsetup{font=footnotesize,skip=2pt} % 図キャプション上の空き
  \captionsetup[sub]{font=footnotesize,skip=1pt} % subcaption上の空き
  \setlength{\tabcolsep}{3pt} % 列間（左右の間）
  \renewcommand{\arraystretch}{0} % 行のデフォ伸びを抑える

  \begin{tabular}{@{}cc@{}}
    \subcaptionbox{LavaCrossing\label{fig:lava}}{%
      \includegraphics[width=.4\textwidth,trim=8 6 8 6,clip]{figures/rl/lava-retry-4env-bars.pdf}} &
    \subcaptionbox{DoorKey\label{fig:doorkey}}{%
      \includegraphics[width=.4\textwidth,trim=8 6 8 6,clip]{figures/rl/doorkey-retry-4env-bars.pdf}} \\
    \subcaptionbox{MultiRoom\label{fig:multiroom}}{%
      \includegraphics[width=.4\textwidth,trim=8 6 8 6,clip]{figures/rl/multiroom-retry-4env-bars.pdf}} &
    \subcaptionbox{All tasks\label{fig:alltask}}{%
      \includegraphics[width=.4\textwidth,trim=8 6 8 6,clip]{figures/rl/alltasks-ID_OOD-avg-bars.pdf}}
  \end{tabular}
  \vspace{2mm}
  \caption{Success rates on \Minigrid tasks, averaged over 5 random seeds. Error bars denote the standard deviation across seeds. Our model(\method) consistently matches or outperforms strong sequence-model baselines and achieves superior average performance across all tasks.}
  \label{fig:results-minigrid}
\end{figure*}



\begin{figure*}[t]
  \centering
  \begin{tabular}{cc}
    \begin{minipage}[c]{0.38\textwidth}
      \centering
      \includegraphics[width=\linewidth]{figures/dyck/acc_id.pdf} \\
      \includegraphics[width=\linewidth]{figures/dyck/acc_ood.pdf}
    \end{minipage}
    & 

    \begin{minipage}[c]{0.56\textwidth}
      \centering
      \includegraphics[width=\linewidth]{figures/dyck/energy.pdf}
    \end{minipage}
  \end{tabular}
    \caption{Dyck results. \textbf{Left:} Token-wise prediction accuracy of Dyck sequences, plotted against length on ID (top) and OOD (bottom).
    The shaded range indicates the sequence lengths used in training.
    The ID strings are randomly generated under the constraint of bracket-depth $\le5$. For the OOD setting, we use 1-regular runs (see Figure~\ref{fig:dyckexample}).  
    \textbf{Right:} An energy trace (See \eqref{eq:energy}) for the first and second layers of hierachical version of \eqref{eq:FastSlow} during a $5$-regular run, aligned with the input sequence (shown at the top of the plot).  
    The energy of the first‑layer spikes with the arrival of a new bracket-\emph{type}, and then settles to the level specific to it. 
    The energy of the second‑layer is organized by bracket-\emph{depth}. 
    The dashed lines indicate the token arrival times.
    }
    \label{fig:dyck-acc-energy}
\end{figure*}


\subsection{Structural components of \eqref{eq:FastSlow}:  $T$ and weight sharing} 

We conducted ablative studies to validate the importance of $T>1$ and weight sharing, which are two essential components of \ref{eq:FastSlow}.  
In accordance to our intuition that longer recurrent thinking helps between observations, we verify that larger $T$ tends to promote the OOD performance, and that weight sharing is also crucial for benefitting from larger $T$. 

\paragraph{Effect of fast-loop iterations}
The number of fast inner-loop iterations ($T$) controls how many recurrent updates occur between successive observations (Eq.~\ref{eq:FastSlow}). 
To investigate whether the model benefits from longer recurrence, we conducted experiments with varying values of $T$ at training while keeping all other components fixed. 
As shown in Figure~\ref{fig:maze_Ttrain}, OOD accuracy improves monotonically as $T$ increases, with gains saturating beyond $T=8$. 
Larger $T$ generally promotes better capturing of the stream dynamics that generalizes OOD.
\maso{See Figure \ref{fig:t-scaling} for the test time scaling.}


\paragraph{Effect of weight sharing (recurrence) in the fast loop.}
Our fast module applies the same update rule repeatedly for $T$ inner steps; that is, it is \emph{recurrent} in the way that it is \emph{weight-shared} across fast iterations.
To investigate the importance of this structure, we replaced it with an \emph{unrolled} residual stack of $T$ distinct layers, while keeping the overall fast--slow interface unchanged.
The results in Table~\ref{tab:ablation_weightshare} show that weight sharing is crucial for OOD generalization: with the same inner-loop budget ($T = 5$), the non-recurrent $5$-layer stack reduces OOD accuracy from approximately $0.6$ to approximately $0.5$.
Increasing depth without sharing does not recover this performance; a $10$-layer unshared stack further degrades OOD accuracy to approximately $0.45$, even after tuning the learning rate.
These results support the design choice of looped recurrence is effective in our \method mechanism of \eqref{eq:FastSlow}.

\begin{table}[t]
\centering
\begin{tabular}{c c c c c}
\toprule
Layers ($T$) & Weight Sharing & Param. (M) & ID Acc & OOD Acc \\
\midrule
5  & ON & 1.16 & $0.968 \pm 0.001$ & $0.612 \pm 0.019$ \\
5  & OFF  & 2.38 & $0.913 \pm 0.059$ & $0.509 \pm 0.098$ \\
10 & OFF & 3.90 & $0.775 \pm 0.320$ & $0.445 \pm 0.164$ \\
\bottomrule
\end{tabular}
\caption{Recurrent-structure ablation on the maze task. When the ``Weight Sharing'' is ON, the model computes $T$ computations in the loop with the same weights. When the ``Weight Sharing'' is OFF,  distinct $T$ layers are being used without recurrence.}
\label{tab:ablation_weightshare}
\end{table}





\begin{wrapfigure}{r}{0.5\textwidth}
    \centering
    \vspace{-\baselineskip}  % optional: tightens vertical spacing
    \includegraphics[width=0.43\textwidth]{figures/maze_VSTtrain.pdf}
\caption{The plot of $T_{train}$ against OOD performance.   
\maso{PLEASE FILL IN THE CLEANER VERSION OF THE PLOT, NUMBERS ARE IN table hat has been commented out(merged)} } 
    \label{fig:maze_Ttrain}
\end{wrapfigure}



% Table~\ref{tab:ablation_recurrentcore} reports mean~$\pm$~std over three seeds for validation accuracy on ID ($19 \times 19$) and OOD ($39 \times 39$) mazes.
% Without weight sharing, increasing the number of layers from $5$ to $10$ degrades OOD performance (from $0.509$ to $0.445$).
% This trend contrasts with that of the recurrent model, in which increasing the number of inner-loop steps $T$ improves OOD accuracy.
% In short, increasing depth without sharing degrades OOD generalization, whereas increasing the number of recurrent updates $T$ in the shared model improves it: simply stacking more independent layers does not reproduce the benefits of a recurrent, weight-shared model.
% \maso{Figure \ref{fig:t-scaling} NOT mentioned yet} 



% \paragraph{Results}
% Table~\ref{tab:ablation_recurrent_core}
% reports mean~$\pm$~std over three seeds for validation ID ($19{\times}19$) and OOD ($39{\times}39$) mazes.
% Without weight sharing, increasing the number of layers from $5$ to $10$ degrades OOD performance (from $0.509$ to $0.445$). 
% This trend contrasts with the recurrent model, where increasing the number of inner-loop steps $T$ improves OOD accuracy. 
% Increasing depth without sharing degrades OOD generalization, whereas increasing the number of recurrent updates $T$ in the shared model improves it.
% Simply stacking more independent layers does not reproduce the same benefits of a recurrent, weight-shared model. 



% \begin{table}[ht!]
% \centering
% \small
% \caption{Results on the maze task, reported as mean~$\pm$~std over $3$ seeds. The $\text{Layers} = 1$ rows show how our recurrent structure with weight sharing performs as a function of $T_{\text{train}}$, the number of inner-loop iterations during training. The $\text{Layers} > 1$ rows show the corresponding results for multi-layer networks without weight sharing.}
% \label{tab:maze_T_and_sharing_merged}
% %\resizebox{0.6\columnwidth}{!}{%
% \begin{tabular}{cc r @{$\,\pm\,$} l}
% \toprule
% Layers & $T_{\text{train}}$ & \multicolumn{2}{c}{OOD Acc.} \\
% \midrule
% \multirow{6}{*}{1} & 1  & 0.306 & 0.135 \\
%                    & 2  & 0.431 & 0.186 \\
%                    & 4  & 0.595 & 0.036 \\
%                    & 5  & 0.612 & 0.019 \\
% %                   & 8  & \bfseries 0.673 & \bfseries 0.006 \\
%                    & 8  &  0.673 & 0.006 \\
%                    & 16 & 0.673 & 0.032 \\
% \midrule
% 5                  & \multirow{2}{*}{1}  & 0.509 & 0.098 \\
% 10                 &                     & 0.445 & 0.164 \\
% \bottomrule
% \end{tabular}%
% %}
% \end{table}

% \begin{table}[t]
% \centering
% \caption{Recurrent-structure ablation on the maze task. When ``Weight Sharing'' is Yes, the model performs $T$ computations in the loop with the same weights. When ``Weight Sharing'' is No, $T$ distinct layers are used without recurrence.}
% \label{tab:ablation_recurrent_core}
% \begin{tabular}{c c c c c}
% \toprule
% Layers ($T$) & Weight Sharing & Param.~(M) & ID Acc. & OOD Acc. \\
% \midrule
% 5  & Yes & 1.16 & $0.968 \pm 0.001$ & $0.612 \pm 0.019$ \\
% 5  & No  & 2.38 & $0.913 \pm 0.059$ & $0.509 \pm 0.098$ \\
% 10 & No  & 3.90 & $0.775 \pm 0.320$ & $0.445 \pm 0.164$ \\
% \bottomrule
% \end{tabular}
% \end{table}







\section{Choice of the recurrent Core \core} 

\maso{Memo: Core ablation goes HERE, Waiting for Results: Figure \ref{fig:module-ablation} would be replaced with more comprehensive table, etc. This section needs to be rich}

Table \ref{tab:ablation_recurrent_core} compares the OOD generalization ability of the mechanism of \eqref{fig:fastslowTask} with various choices of core, tested on \Localmaze. 
\begin{itemize}
\item CNN Core
\item Linear Attention Core
\item Mamba Core
\item LSTM Core
\item $\core_{TF}$
\item $\core_{\akorn}$ (\ref{app:impl-J})
\end{itemize}
Expected contents 
\begin{itemize}
\item We observed that most important component to be included in $\core$ was ... 
\item Interestingly \eqref{eq:FastSlow} with other cores such as XX and YY were able too
\item Combination was very important 
\item There was a sensitivity especially for ZZZZ
\end{itemize}

\begin{figure}[ht!]
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/maze/id-main-reccurence.pdf}
        \caption{ID accuracy ($19 \times 19$).}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/maze/ood-main-reccurence.pdf}
        \caption{OOD accuracy ($39 \times 39$).}
    \end{subfigure}
    \caption{\maso{INCOMPLETE} Comparison of different fast modules in the maze task.
    We replaced the AKOrN fast module with either a Transformer block or an LSTM while keeping the remaining architecture and training protocol fixed. 
    The results suggest that a transformer can also serve as a recurrent core in our fast-slow modeling. }
    \label{fig:module-ablation}
\end{figure}




\section{Qualitative analysis: Emergent structure in latents}
Interestingly, through learning the prediction task on the Dyck language, our model discovers latent reasoning that aligns with the structural organization of the input.
Recall that for the recurrence used in our experiments (Section~\ref{sec:recurrence_structure}), there exists an energy-like scalar that reflects the organizational level of the state.
We show the evolution of this energy in Figure~\ref{fig:dyck-acc-energy}, and the evolution of the latent in Figure~\ref{fig:dyck-pca}.
The energy of $X^{(1)}$ spikes upon the arrival of a new token and then stabilizes at a level that depends on the bracket type and on whether the current token is opening or closing.
In contrast, the energy of $X^{(2)}$ is largely insensitive to bracket identity and is instead organized by stack \emph{depth}.
This qualitative shift in energy organization indicates that the second fast process abstracts away from token identity and operates at a higher structural level.
%
PCA projections of the latents for both $X^{(1)}$ and $X^{(2)}$ support this interpretation: the state trajectories form a crisp, spring-shaped manifold indexed by stack depth that remains coherent over long horizons.
This structured organization of the learned latent space is consistent with the observation of \citet{ouro2025} that looped models tend to produce interpretable reasoning traces.
This behavior stands in stark contrast to that of Mamba (Figure~\ref{fig:dyck-pca-mamba}).

We observe a similarly clear emergent structure in the latent space of our learned model on the \Minigrid experiment.
Fluctuations in the energy value reflect the agent's level of ``frustration''; for example, the energy responds when the agent's vision changes beyond a certain threshold (Figure~\ref{fig:doorkey_energy}).
Figure~\ref{fig:doorkey_pca} shows PCA-projected latent state transitions for DoorKey: irrespective of the trajectory, the model organizes its representations around key events such as ``key pickup'', ``door opening'', and ``goal discovery''.

These observations are consistent with recent findings that looped attention-based computation converges to cyclic fixed points in latent space \citep{blayney2026mechanistic}, and that continuous-time attention dynamics exhibit metastable clustering \citep{geshkovski2024dynamic, geshkovski2025mathematical}.
Importantly, these emergent structures serve as a scaffold for \emph{reusable} representations across the evolution of the stream: once formed, representations characterized by task-relevant properties such as stack depth, bracket type, and key events are reused repeatedly by the trajectory along the stream.
This suggests that the structural properties discovered in the qualitative and theoretical studies above, namely the formation of attractors, play an essential role in allowing the model to discover the generative rules of the stream.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.4\linewidth]{figures/rl/energy_doorkey.pdf}
    \includegraphics[width=0.4\linewidth]{figures/rl/visualize_doorkey.png}

    \caption{
     (Left) Energy traces (See \ref{sec:fastslow}) along an episode in the DoorKey-16x16 (OOD) environment. \textbf{Top:} Event history along the trajectory. Markings correspond to events.  The red cross marks the changes in agent's view. \textbf{Bottom:} Energy trajectories.  (Right)     Latent state trajectories of 30 episodes for DoorKey-16x16 (OOD) environment, visualized by PCA.
    Observe that important events are forming trajectory-independent clusters.  }
    \label{fig:doorkey_visual}
\end{figure}

% \begin{figure}[t]
%     \centering
%     \caption{
%     Latent state trajectories of 30 episodes for DoorKey-16x16 (OOD) environment, visualized by PCA.
%     Observe that important events are forming trajectory-independent clusters.}
%     \label{fig:doorkey_pca}
% \end{figure}


\begin{figure*}[tb]
  \centering
\begin{minipage}{0.85\textwidth}
\centering
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}ccc@{}}
\begin{subfigure}[b]{0.32\linewidth}
  \includegraphics[width=\linewidth]{figures/dyck/pca_1st.pdf}
  \caption{Ours: 1st-layer states}
\end{subfigure}
&
\begin{subfigure}[b]{0.32\linewidth}
  \includegraphics[width=\linewidth]{figures/dyck/pca_2nd.pdf}
  \caption{Ours: 2nd-layer states}
\end{subfigure}
&
\begin{subfigure}[b]{0.32\linewidth}
  \includegraphics[width=\linewidth]{figures/dyck/pca_mamba.pdf}
  \caption{Mamba: last-layer states}
  \label{fig:dyck-pca-mamba}
\end{subfigure}
\end{tabular*}
\end{minipage}
  \caption{Comparison of latent trajectories of a $5$-regular run of length 2,560, visualized via PCA; $\circ$ marker indicates an open bracket and $\times$ marker indicates a close bracket. 
  (a) Trajectory of the first layer latents of our model (\method). The color of the node indicates the bracket type. 
  (b) Trajectory of the second layer latents of our model (\method). They are organized by stack depth (color) and opening/closing state. 
  (c) Mamba's state trajectories at its last layer. They form a diffuse, overlapping cloud with frequent crossings and weaker organization. 
  % \rev{Comparison of latent state trajectories on a $5$-regular run of length 2,560. (a) PCA of the first-layer latents at the last fast step shows a star-shaped structure whose endpoints correspond to different opening brackets (color indicates bracket type). (b) The second-layer latents remain organized by stack depth (color) and opening/closing state ($\circ$ for open, $\times$ for close), indicating coherent, length-general computation. (c) Mamba's state trajectories at the last layer form a diffuse, overlapping cloud with frequent crossings and weaker organization by stack depth.  Mamba generalizes weaker in OOD domain.}
  }
  \label{fig:dyck-pca}
\end{figure*}




% \begin{itemize}
% % \item Descrpition of the environments;  localMaze, RL, Dyck, etc 
% \item Ablation: Resets (Appendix) 
% \item Hyperparam? : (Appendix) 
% \item Ablation: Loop Numbers
% \item Ablation: Core choices
% \begin{itemize}
% \item AttnCores 
% \item Weight Sharing Cores
% \item Nonlinearity 
% \item Normalization 
% \item Delta From AKOrN 
% \end{itemize}

% \end{itemize}




% \begin{figure}[b!]
%     \begin{minipage}[t]{\columnwidth}
%     \vspace{0pt}
%         \centering
%         % (a)
%         \begin{subtable}[t]{0.48\columnwidth}
%             \centering
%             \includegraphics[width=\columnwidth]{figures/maze/id-smaple.png}
%             \caption{In-distribution ($19\times 19$)}
%             \label{fig:sample-id}
%         \end{subtable}
%         \hfill
%         % (b)
%         \begin{subfigure}[t]{0.48\columnwidth}
%             \centering
%             \includegraphics[width=\columnwidth]{figures/maze/ood-sample.png}
%             \caption{OOD ($39\times 39$)}
%             \label{fig:sample-ood}
%         \end{subfigure}
    
%         \captionof{figure}{
%         \Localmaze examples. Models are trained on small mazes (a) and evaluated on larger mazes (b). The green cell denotes the start, the red cell denotes the goal, and the observation is always limited to a $7\times 7$ region centered on its current position.
%             %Examples of maze environments. (a) In-distribution maze ($19\times19$). (b) Out-of-distribution maze ($39\times39$).
%         }
%         \label{fig:maze-sample}
%     \end{minipage}
% \end{figure}

% \section{Experiments}\label{sec:exp}

% We conducted a series of experiments to assess our model’s ability to dynamically integrate sequential inputs into its recurrent process in support of correct inference.
% We selected tasks that fundamentally require the model to iteratively and selectively identify task-relevant information from an evolving input sequence, and to consolidate it by continuously integrating this information into the latent state.

% We first present results on \Localmaze and Dyck tasks, both of which provide supervision in the form of correct answers. In these settings, the model can retrospectively infer which parts of the input are irrelevant to the correct underlying structure of the data.
% We additionally consider more challenging reinforcement learning tasks on MiniGrid. In these online settings, the model cannot directly compute the correct regret or value signal from immediate rewards, and therefore must learn indirectly how to integrate episodic information as it explores the environment.

% \paragraph{Hyperparameter}
% For the maze and Dyck tasks, we first identified a common set of training hyperparameters—specifically the number of epochs, batch size, and learning rate—for which validation performance converged across all baselines. After fixing these shared settings, we further tuned model-specific hyperparameters (e.g., learning rate and hidden dimensionality) independently for each baseline in order to maximize validation performance.
% %
% For the MiniGrid experiments, we adopted the same hyperparameters for all baselines as in \citet{ivan2025benchnetrl}, while tuning the hyperparameters of our proposed method separately.
% Also see Appendix (Tables~\ref{tab:hparams-merged} and \ref{tab:model-hparams-maze-minigrid}).


% \begin{figure*}[t]
%     \centering
%     \begin{subfigure}[b]{0.49\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/maze/id-main.pdf}
%         \caption{ID mazes ($19\times19$)}
%         \label{fig:maze-id}
%     \end{subfigure}
%     \hfill
%     %\hspace{1em}
%     \begin{subfigure}[b]{0.49\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/maze/ood-main.pdf}
%         \caption{OOD mazes ($39\times39$)}
%         \label{fig:maze-ood}
%     \end{subfigure}
%     \caption{Accuracy comparison of our model(\method) with baselines on the maze task. 
%     Our model(\method) shows substantially better OOD generalization. 
%     % \kohei{\texttt{Ours(V)} uses no auxiliary memory, \texttt{Ours(I)} uses internal memory, \texttt{Ours(E)} uses external memory, and \texttt{Ours(IE)} uses both.}
%     }
%     \label{fig:results-maze}
% \end{figure*}

% \subsection{\Localmaze} \label{sec:maze}

% The goal of this task is to infer the shortest path from the start to the end, while receiving a stream of egocentric observations from a navigator exploring the maze.  
% In this task, the information corresponding to dead-end paths is naturally task-irrelevant.
% In order for the model to be able to generalize its inference capability to OOD mazes of large size, the model must learn to efficiently integrate the task-relevant information and iteratively consolidate its hypothesis about the shortest path.

% More specifically, the model in this task is given a sequence of local, cropped $7\times 7$ neighborhood images $O_s$ corresponding to the egocentric observations of a navigator agent that explores the maze following the right-hand rule (the model has no control over the navigator).
% The navigator streams egocentric observations until the goal is reached. 
% The decoded output of the model is a sequence of movements (\texttt{up, down, left, right, pause}) corresponding to the estimated shortest path. 
% Depending on the geometry of the maze, the length of the observation sequence $S$ naturally varies across samples. 
% As a supervisory signal to be compared against the decoded output, we provide the model, at the end of each episode, with the true shortest path for the maze, represented in the same format. 
% We evaluate accuracy using a binary exact-match criterion on the entire predicted action sequence, after removing all \texttt{pause} tokens from both the prediction and the ground-truth shortest path.





% \paragraph{Setup}
% The mazes are generated randomly. 
% During training, they are of size $19 \times 19$. 
% We evaluate the model’s generalization on out-of-distribution (OOD) mazes of size $39 \times 39$.
% Figure~\ref{fig:maze-sample} shows examples of mazes for both the in-distribution (ID) and OOD settings.
% In the OOD setting, the observation sequence length $S$ tends to be naturally larger.

% We evaluate seven models on the maze task: LSTM, Transformer (TF), Mamba-2~\citep{dao2024transformers}, looped TF~\citep{Looped}, S5~\citep{smith2022simplified}, CTM~\citep{CTM}, and our model. Our dataset contains 45,000 training and 5,000 validation examples, in which training mazes are generated so that shortest‑path lengths are uniformly distributed.
% %We assess performance in both ID and OOD scenarios.
% For the default setting, we set $T=5$.
% Hyperparameters are tuned on the ID validation set and used unchanged for OOD evaluation. See Appendix~\ref{app:maze-details} for details. We report the mean $\pm$ sd over three seeds.


% % \paragraph{Designing \texorpdfstring{$J_t(X(t), C(s(t)))$}{J_t(X(t), C(t))} with Internal Memory}

% % Let the fast-time index be $t=0,1,2,\dots$ and the slow observation index be $s(t)=\lfloor t/T\rfloor$.
% % At each fast step, update the inner-loop and the internal memory causally:
% % \begin{align}
% % s_t &= \psi\!\bigl(X_t,\,C(s(t))\bigr), \\
% % h_{t+1} &= \mathrm{GRU}\!\bigl(s_t,\,h_t\bigr),
% % \label{eq:int-mem}
% % \end{align}
% % where $\psi$ is any function of the inner-loop state $X_t$ and the observation $C(s(t))$.

% % Define the objective at fast time $t$ as a continuous mapping of the internal memory:
% % \begin{align}
% % J_t \;\equiv\; J\!\bigl(\,\cdot\,;\,h_t,\,C(s(t))\bigr) \;:=\; \Phi(h_t)\,,
% % \end{align}
% % and constrain $\Phi$ to be Lipschitz (e.g., via spectral normalization or $1{\times}1$ convolutions). Then, for some constant $L>0$,
% % \begin{align}
% % \bigl\|J_{t+1}-J_t\bigr\| \;\le\; L\,\bigl\|h_{t+1}-h_t\bigr\|\,,
% % \label{eq:Lipschitz}
% % \end{align}
% % so $J_t$ evolves smoothly over fast time.


% \begin{table}[t]
% \centering
% \small
% \caption{
% Results of the maze task, represented in the format of  Mean $\pm$ std over 3 seeds. Layer=1 results describe how our recurrent structure with weight sharing performs with respect to $T_{train}$, the number of inner loop iterations in training.  
% $\text{Layers} > 1$ represent the results of multi-layer networks without weight sharing. 
% % \rev{Maze task results. Rows with $\text{Layers}=1$ correspond to the recurrent structure with weight sharing, where $T$ denotes the number of inner-loop iterations. Rows with $\text{Layers} > 1$ represent standard feedforward networks without weight sharing ($T=1$). Mean $\pm$ std over 3 seeds.}
% }
% \label{tab:maze_T_and_sharing_merged}
% %\resizebox{0.6\columnwidth}{!}{%
% \begin{tabular}{cc r @{$\,\pm\,$} l}
% \toprule
% Layers & $T_{train}$ & \multicolumn{2}{c}{OOD Acc.} \\
% \midrule
% \multirow{6}{*}{1} & 1  & 0.306 & 0.135 \\
%                    & 2  & 0.431 & 0.186 \\
%                    & 4  & 0.595 & 0.036 \\
%                    & 5  & 0.612 & 0.019 \\
% %                   & 8  & \bfseries 0.673 & \bfseries 0.006 \\
%                    & 8  &  0.673 & 0.006 \\
%                    & 16 & 0.673 & 0.032 \\
% \midrule
% 5                  & \multirow{2}{*}{1}  & 0.509 & 0.098 \\
% 10                 &                     & 0.445 & 0.164 \\
% \bottomrule
% \end{tabular}%
% %}
% \end{table}

% \paragraph{Results}

% Our model significantly outperforms all baselines on the maze task. As shown in Figure \ref{fig:results-maze}, it achieves near-perfect accuracy on the $19\times19$ (ID) mazes and, crucially, demonstrates strong generalization to unseen $39\times39$ mazes with approximately $60\%$ accuracy. In contrast, the baseline models all fail to generalize.

% % \begin{figure*}[h]
% %     \centering
% %     \begin{subfigure}[b]{0.49\textwidth}
% %         \includegraphics[width=\textwidth]{figures/maze/id-main.png}
% %         \caption{ID mazes ($19\times19$)}
% %         \label{fig:maze-id}
% %     \end{subfigure}
% %     \hfill
% %     \begin{subfigure}[b]{0.49\textwidth}
% %         \includegraphics[width=\textwidth]{figures/maze/ood-main.png}
% %         \caption{OOD mazes ($39\times39$)}
% %         \label{fig:maze-ood}
% %     \end{subfigure}
% %     \caption{Performance comparison of our model with baselinse on the Maze task. %Comparison of our model with baselines on (a) in-distribution ($19\times19$ mazes) and (b) out-of-distribution ($39\times39$ mazes). 
% %     Our model demonstrates superior generalization capability in the OOD setting.}
% %     \label{fig:results-maze}
% % \end{figure*}


% % \begin{figure*}[t]
% %     \centering
% %     \begin{subfigure}[b]{\columnwidth}
% %         \includegraphics[width=\columnwidth]{figures/maze/id-main.pdf}
% %         \caption{ID mazes ($19\times19$)}
% %         \label{fig:maze-id}
% %     \end{subfigure}
% %     \hfill
% %     \begin{subfigure}[b]{\columnwidth}
% %         \includegraphics[width=\columnwidth]{figures/maze/ood-main.pdf}
% %         \caption{OOD mazes ($39\times39$)}
% %         \label{fig:maze-ood}
% %     \end{subfigure}
% %     \caption{Accuracy comparison of our model with baselines on the maze task. 
% %     Our model shows substantially better OOD generalization. 
% %     % \kohei{\texttt{Ours(V)} uses no auxiliary memory, \texttt{Ours(I)} uses internal memory, \texttt{Ours(E)} uses external memory, and \texttt{Ours(IE)} uses both.}
% %     }
% %     \label{fig:results-maze}
% % \end{figure*}



% \paragraph{Effect of fast-loop iterations}
% The number of fast inner-loop iterations ($T$) controls how many recurrent updates occur between successive observations (Eq.~\ref{eq:FastSlow}). 
% To investigate whether the model benefits from longer recurrence, we conducted experiments with varying values of $T$ while keeping all other components fixed. 
% As shown in Table~\ref{tab:maze_T_and_sharing_merged}, OOD accuracy improves monotonically as $T$ increases, with gains saturating beyond $T=8$. 

% \paragraph{Effect of weight sharing (recurrence) in the fast loop}
% Our fast module applies the same update rule repeatedly for $T$ inner steps, i.e., it is \emph{recurrent} or \emph{weight-shared} across fast iterations. 
% To investigate the importance of this recurrent structure, we replaced it with an \emph{unrolled} residual stack of $T$ distinct layers, while keeping the overall fast--slow interface unchanged. 
% The results (Table~\ref{tab:maze_T_and_sharing_merged})
% show that weight sharing is crucial for OOD generalization: with the same inner-loop budget ($T{=}5$), the non-recurrent 5-layer stack reduces OOD accuracy from approximately $0.6$ to approximately $0.5$. 
% Increasing depth without sharing does not recover this performance: a 10-layer unshared stack further degrades OOD accuracy to approximately $0.45$, even after adjusting the learning rate. 
% These results support our design choice of a recurrent fast module.
% Please also see \ref{app:ablation_recurrent}.

% %The full details are in the Appendix~\ref{app:ablation_recurrent}.





% % \begin{table}[t]
% % \centering
% % \small
% % \setlength{\tabcolsep}{6pt}
% % \begin{tabular}{c c}
% % \toprule
% % Training-time $T$ & OOD Acc.\\
% % \midrule
% % 1  & $0.306 \pm 0.135$ \\
% % 2  & $0.431 \pm 0.186$ \\
% % 4  & $0.595 \pm 0.036$ \\
% % 8  & $\mathbf{0.673 \pm 0.006}$ \\
% % 16 & $0.673 \pm 0.032$ \\
% % \bottomrule
% % \end{tabular}
% % \caption{OOD accuracy on the maze task, varying fast inner-loop iterations $T$ used during training (mean $\pm$ std over 3 seeds). Increasing $T$ monotonically improves OOD generalization.}
% % \label{tab:T_train_scaling}
% % \end{table}

% % \begin{table}[t]
% % \centering
% % \small
% % \caption{OOD accuracy on the maze task, varying fast inner-loop iterations $T$ used during training (mean $\pm$ std over 3 seeds). Increasing $T$ monotonically improves OOD generalization.}
% % \label{tab:T_train_scaling}
% % \begin{tabularx}{\linewidth}{c Y}
% % \toprule
% % Training-time $T$ & OOD Acc.\\
% % \midrule
% % 1  & $0.306 \pm 0.135$ \\
% % 2  & $0.431 \pm 0.186$ \\
% % 4  & $0.595 \pm 0.036$ \\
% % 8  & $\mathbf{0.673 \pm 0.006}$ \\
% % 16 & $0.673 \pm 0.032$ \\
% % \bottomrule
% % \end{tabularx}
% % \end{table}


% % \subsection{Dyck-$(k,m)$}\label{sec:dyck}

% % \begin{figure}[t]
% % \vspace{-8pt}
% % \begin{subfigure}{1\textwidth}
% %   \centering  \includegraphics{figures/dyck/example_id.pdf}
% %   \vspace{-5pt}
% %   \caption{ID (random pattern)}
% %   \vspace{5pt}
% % \end{subfigure}
% % %-----------------(b)-----------------%
% % \begin{subfigure}{1\textwidth}
% %   \centering
% %   \includegraphics{figures/dyck/example_ood.pdf}
% %   \vspace{-5pt}
% %   \caption{OOD (1-regular run)}
% %   \vspace{5pt}
% % \end{subfigure}
% % \caption{Dyck language examples. 
% % %\rev{In 1-regular runs, the first open brackets (highlighted in red) reappear as prediction targets arbitrarily far into the sequence, testing the ability to retain information.}
% % (a) When the stack is empty, ``$*$'' is the next predicted token. 
% % (b) The predictor must remember ``['' forever while ``()'' continues in the input.}
% % \label{fig:dyckexample}
% % \end{figure}

% \begin{figure}[t]
% \begin{minipage}{\columnwidth}
%     \vspace{-.5em}
%     \begin{subfigure}{0.49\linewidth}
%     \hspace{-7mm}\includegraphics[width=1.2\linewidth]{figures/dyck/example_id.pdf}
%       \caption{ID (random pattern)}
%       \label{fig:dyck-id}
%     \end{subfigure}
%     \begin{subfigure}{0.49\linewidth}
%       \hspace{-7mm}\includegraphics[width=1.2\linewidth]{figures/dyck/example_ood.pdf}
%       \caption{OOD (1-regular run)}
%       \label{fig:dyck-ood}
%     \end{subfigure}
% \end{minipage}

% \caption{
% Dyck examples. 
% (a) The target at position $s$ is the token that closes the most recent unclosed bracket in the prefix up to $s$. When the stack is empty, ``$*$'' is predicted. 
% (b) In a $1$-regular run, the predictor is required to output the token that closes the first open bracket (e.g., ``$[$'') at every odd step, while remembering this unresolved bracket for as long as the sequence continues.}
% % \rev{In 1-regular runs, the first open brackets (highlighted in red) reappear as prediction targets arbitrarily far into the sequence, testing the ability to retain information.}
% % (a) When the stack is empty, ``$*$'' is the next predicted token. 
% % (b) The predictor must remember ``['' forever while ``()'' continues in the input.}
% \label{fig:dyckexample}
% \end{figure}



% \subsection{Dyck-$(k, m)$} \label{sec:dyck}

% We also experimented with the symbolic generalization task on Dyck-$(k,m)$~\citep{hewitt2020rnns}, with $k$ bracket types and maximum depth $m$. 
% Dyck is a stack-related task that heavily requires long-range lookup as well as iterative consolidation of the current stack structure, and it is the task referred to in the introduction. 
% We set $m=5$ and $k=30$.

% Given a streaming input of brackets as ``[\{([(('',  the goal is to sequentially predict the next bracket token that closes the most recent \emph{unclosed} bracket.
% For example, when the input sequence up to $s=4$ is ``\verb|({[]|'', the prediction at $s=4$ should be ``\}''. 
% When there is no bracket to close, the prediction should be ``*''; also see Figure~\ref{fig:dyckexample}. 
% % See \ref{app:dyck-details} for more details.
% % \footnote{\citet{hewitt2020rnns} originally formulated this task as standard next-token prediction. 
% %  However, because there are multiple valid choices for the type of the next open bracket, the task is not deterministic when formulated as pure next-token prediction. 
% % To eliminate this source of indeterminacy in accuracy evaluation, we restrict the predictor to output only the closing bracket.}


% % Given a streaming input of brackets $\{O_r \mid r < s\}$ (e.g., a sequence such as ``[, \{''), the goal is to sequentially predict the next bracket token $\hat{O}_s$ that closes the most recent \emph{unclosed} bracket.
% % \footnote{\citet{hewitt2020rnns} originally formulated this task as standard next-token prediction. 
% % However, because there are multiple valid choices for the type of the next open bracket, the task is not deterministic when formulated as pure next-token prediction. 
% % To eliminate this source of indeterminacy in accuracy evaluation, we restrict the predictor to output only the closing bracket.}
% % For example, when the input sequence up to $s=5$ is ``\verb|({[]|'', the prediction $\hat{O}_5$  should be ``)''.  
% % When there is no bracket to close in the previous tokens, the prediction should be ``*''; see Figure~\ref{fig:dyckexample}.  
% % Predictions are made sequentially at every $s$. 
% % For instance, if the sequence of \textit{input tokens} $O_{< 5}$ up to $s=4$ is ``\verb|()[{|'', the output sequence of \textit{predicted tokens}  $\hat{O}_{<5}$ is ``\verb|)*]}|''.


% The streaming sequence of brackets is analogous to an ever-growing stack of jobs, where the depth at time $s$ corresponds to the number of remaining brackets to close. 
% By design, this task requires the model to remember all unclosed brackets for as long as the sequence continues. 
% For example, for sequences of the form ``\verb|[()()()()|$\cdots$'' in Figure~\ref{fig:dyckexample}, the model must remember the unclosed ``\verb|[|'' as long as the sequence continues. 
% See \ref{app:dyck-details} for more details.

% \begin{figure*}[t]
%   \centering
%   \begin{tabular}{cc}
%     \begin{minipage}[c]{0.38\textwidth}
%       \centering
%       \includegraphics[width=\linewidth]{figures/dyck/acc_id.pdf} \\
%       \includegraphics[width=\linewidth]{figures/dyck/acc_ood.pdf}
%     \end{minipage}
%     & 

%     \begin{minipage}[c]{0.56\textwidth}
%       \centering
%       \includegraphics[width=\linewidth]{figures/dyck/energy.pdf}
%     \end{minipage}
%   \end{tabular}
%     \caption{Dyck results. \textbf{Left:} Token-wise prediction accuracy of Dyck sequences, plotted against length on ID (top) and OOD (bottom).
%     The shaded range indicates the sequence lengths used in training.
%     The ID strings are randomly generated under the constraint of bracket-depth $\le5$. For the OOD setting, we use 1-regular runs (see Figure~\ref{fig:dyckexample}).  
%     \textbf{Right:} An energy trace (See \ref{sec:choice}) for the first and second layers during a $5$-regular run, aligned with the input sequence (shown at the top of the plot).  
%     The energy of the first‑layer spikes with the arrival of a new bracket-\emph{type}, and then settles to the level specific to it. 
%     The energy of the second‑layer is organized by bracket-\emph{depth}. 
%     The dashed lines indicate the token arrival times.
%     }
%     \label{fig:dyck-acc-energy}
% \end{figure*}


% \paragraph{Setup}

% For the ID dataset, we randomly generate Dyck-$(30,5)$ strings.
% For the OOD dataset, we define a sequence to be an \textit{$n$-regular run} if it has the following structure:  
% (i) it begins with a random sequence of \textit{open} brackets of random length, and  
% (ii) it is followed by an infinite repetition of depth-$n$ openings and depth-$n$ closings.  
% For example, ``\verb|({[([[]](()){{}}|\dots'' is a $2$-regular run, and the one in Figure~\ref{fig:dyckexample} is a $1$-regular run.
% We use $1$-regular run for the OOD evaluation.
% % In general, $1$-regular runs is most difficult because predictions requiring memory of the initial ``\verb|[|'' constitute a higher proportion of the sequence (approximately $1/2$).

% We trained the model on 10{,}000 random strings in an ID dataset of length $\le 40$.  
% For evaluation, the model sequentially predicts on 1{,}000 $n$-regular runs of length up to 2{,}560.  
% Accuracy is computed for the prediction of each bracket.
% %
% We compare our model against LSTM, Transformer, and Mamba-2, which achieved relatively good performance in the maze experiments. 

% Since this task involves a hierarchical structure, we evaluate an extended variant of Eq.~\ref{eq:FastSlow} with two fast processes. 
% Specifically, for $\ell = 0,1,2$, we set $\bX^{(0)}(t) = \bC(t)$ and
% \begin{align*}\small
% \bX^{(\ell)}(t+1) = \Pi\left(\bX^{(\ell)}(t) + \gamma F\!\left(\bX^{(\ell)}(t), \bX^{(\ell-1)}(t)\right)\right)
% \end{align*}
% Predictions are obtained by decoding the last layer's output at each slow-time index $s$.  
% See Appendix~\ref{app:dyck-details} for details.



% \paragraph{Results}

% Figure~\ref{fig:dyck-acc-energy} shows token-level accuracy against the sequence length for both ID and OOD settings. 
% On ID data, all models except the vanilla Transformer extrapolate reasonably well across sequence lengths. 
% In contrast, on the OOD patterns of $1$-regular runs, all baselines eventually fall to the chance level ($0.5$) as the sequence length increases.
% This chance-level behavior corresponds to the cases of failing to predict the token that closes the first open bracket (colored red in Figure~\ref{fig:dyckexample}).
% Our model, however, maintains near $100\%$ accuracy over indefinitely long sequences, indicating that it retains the information of the first opening token while correctly predicting all other subsequent closures. 



% \paragraph{Comparison to LLMs}

% To relate this benchmark to current foundation models, we also compared our model against three frontier LLMs on the same Dyck-$(30,5)$ task (see Figure~\ref{fig:dyck-llms} in the introduction). 
% For the evaluation of our method in this comparative study, we used the model trained with the seed that attained the highest OOD accuracy at length 2,560 in producing Figure \ref{fig:dyck-acc-energy}. 
% In contrast to our model, which is trained only on raw Dyck strings of length $\le 40$, the LLMs are provided with a natural-language prompt describing the ground-truth algorithm that generates the sequence and are instructed to iteratively execute it; see \ref{app:dyck-details} for more details of the setup. 
% Despite their advantage in parameter scale and access to the explicit algorithm, their token-wise accuracy deteriorates as sequence length increases, whereas our model maintains accuracy above $90\%$ on sequences that are two orders of magnitude longer.

% \paragraph{Emergent structure in layerwise energies and latents}

% Interestingly, through learning the prediction task, our model discovers latent reasoning that aligns with the structural organization of the Dyck language. 
% Recall that for the recurrence used in our experiments (Section~\ref{sec:choice}), there exists an energy-like scalar that reflects the organizational level of the state. 
% We show the evolution of this energy in Figure~\ref{fig:dyck-acc-energy}, and the evolution of the latent in Figure~\ref{fig:dyck-pca}.
% %The evolution of this energy is shown in Figure~\ref{fig:dyck-acc-energy}, and the corresponding latent trajectories are shown in Figure~\ref{fig:dyck-pca}.
% %
% The energy of $X^{(1)}$ spikes upon the arrival of a new token and then stabilizes at a level that depends on the bracket type and whether the current token is opening or closing. 
% In contrast, the energy of $X^{(2)}$ is largely insensitive to bracket identity and is instead organized by stack \emph{depth}.
% This qualitative shift in energy organization indicates that the second fast process abstracts away from token identity and operates at a higher structural level.
% %
% PCA projections of the latents for both $X^{(1)}$ and $X^{(2)}$ support this interpretation: the state trajectories form a crisp, spring-shaped manifold indexed by stack depth that remains coherent over long horizons. 
% This structured organization in the learned latent space is similar to the report in 
% \cite{ouro2025} that the looped model tends to produce interpretable reasoning traces.
% This behavior stands in stark contrast to Mamba (Figure~\ref{fig:dyck-pca-mamba}).


% % \begin{wrapfigure}{r}{0.45\textwidth} % r = right, l = left
% %   \centering
% %   \vspace{-10pt} % optional: tweak vertical position
% %   \includegraphics[width=\linewidth]{figures/dyck/llms.pdf}
% %   \caption{\rev{Comparison with LLMs on Dyck. The shaded area indicates the training lengths.}}
% %   \label{fig:dyck-llms}
% % \end{wrapfigure}
% % \begin{figure}[tb]
% %   \centering
% %   \includegraphics[width=0.9\linewidth]{figures/dyck/llms.pdf}
% %   \caption{\rev{Comparison with LLMs on Dyck. The shaded area indicates the training lengths.}}
% %   \label{fig:dyck-llms}
% % \end{figure}
% % %

% %, showing that our model executes the streaming algorithm more reliably beyond the fixed context window.
% %The Dyck comparison therefore probes a regime in which both paradigms in principle admit more computation per input; LLMs through longer reasoning traces up to the token limit, and our model through larger $T$, yet only the proposed fast–slow recurrent architecture behaves as a reliable streaming algorithm executor beyond the fixed context window. 




% % ========= New Figure 8: PCA triptych (layer1, layer2, Mamba) =========
% % \begin{figure*}[tb]
% %   \centering
% %   \begin{subfigure}[b]{0.32\textwidth}
% %     \includegraphics[width=\textwidth]{figures/dyck/pca_1st.pdf}
% %     \caption{Ours: 1st-layer states}
% %     \label{fig:dyck-pca-1st}
% %   \end{subfigure}\hfill
% %   \begin{subfigure}[b]{0.32\textwidth}
% %     \includegraphics[width=\textwidth]{figures/dyck/pca_2nd.pdf}
% %     \caption{Ours: 2nd-layer states}
% %     \label{fig:dyck-pca-2nd}
% %   \end{subfigure}\hfill
% %   \begin{subfigure}[b]{0.32\textwidth}
% %     \includegraphics[width=\textwidth]{figures/dyck/pca_mamba.pdf}
% %     \caption{Mamba: last-layer states}
% %     \label{fig:dyck-pca-mamba}
% %   \end{subfigure}

% %   \caption{\rev{Comparison of latent state trajectories on a $5$-regular run of length 2,560. (a) PCA of the first-layer latents at the last fast step shows a star-shaped structure whose endpoints correspond to different opening brackets (color indicates bracket type). (b) The second-layer latents remain organized by stack depth (color) and opening/closing state ($\circ$ for open, $\times$ for close), indicating coherent, length-general computation. (c) Mamba's state trajectories at the last layer form a diffuse, overlapping cloud with frequent crossings and weaker organization by stack depth.  Mamba generalizes weaker in OOD domain.}}
% %   \label{fig:dyck-pca}
% % \end{figure*}
% \begin{figure*}[tb]
%   \centering
% \begin{minipage}{0.85\textwidth}
% \centering
% \begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}ccc@{}}
% \begin{subfigure}[b]{0.32\linewidth}
%   \includegraphics[width=\linewidth]{figures/dyck/pca_1st.pdf}
%   \caption{Ours: 1st-layer states}
% \end{subfigure}
% &
% \begin{subfigure}[b]{0.32\linewidth}
%   \includegraphics[width=\linewidth]{figures/dyck/pca_2nd.pdf}
%   \caption{Ours: 2nd-layer states}
% \end{subfigure}
% &
% \begin{subfigure}[b]{0.32\linewidth}
%   \includegraphics[width=\linewidth]{figures/dyck/pca_mamba.pdf}
%   \caption{Mamba: last-layer states}
%   \label{fig:dyck-pca-mamba}
% \end{subfigure}
% \end{tabular*}
% \end{minipage}
%   \caption{Comparison of latent trajectories of a $5$-regular run of length 2,560, visualized via PCA; $\circ$ marker indicates an open bracket and $\times$ marker indicates a close bracket. 
%   (a) Trajectory of the first layer latents of our model(\method). The color of the node indicates the bracket type. 
%   (b) Trajectory of the second layer latents of our model(\method). They are organized by stack depth (color) and opening/closing state. 
%   (c) Mamba's state trajectories at its last layer. They form a diffuse, overlapping cloud with frequent crossings and weaker organization. 
%   % \rev{Comparison of latent state trajectories on a $5$-regular run of length 2,560. (a) PCA of the first-layer latents at the last fast step shows a star-shaped structure whose endpoints correspond to different opening brackets (color indicates bracket type). (b) The second-layer latents remain organized by stack depth (color) and opening/closing state ($\circ$ for open, $\times$ for close), indicating coherent, length-general computation. (c) Mamba's state trajectories at the last layer form a diffuse, overlapping cloud with frequent crossings and weaker organization by stack depth.  Mamba generalizes weaker in OOD domain.}
%   }
%   \label{fig:dyck-pca}
% \end{figure*}
% % =====================================================================






% % \begin{figure}[t]
% %     \centering
% %     \begin{subfigure}[b]{0.45\linewidth}
% %         \centering
% %         \includegraphics[width=\linewidth]{figures/dyck/acc_id.pdf}
% %         \caption{ID (Random)}
% %     \end{subfigure}
% %     \hfill
% %     \begin{subfigure}[b]{0.45\linewidth}
% %         \centering
% %         \includegraphics[width=\linewidth]{figures/dyck/acc_ood.pdf}
% %         \caption{OOD ($1$-regular runs)}
% %     \end{subfigure}
% %     \caption{\rev{Dyck token accuracy by length. (a) ID denotes Dyck strings randomly generated under the constraint of depth $\le5$. (b) OOD denotes $1$-regular runs-strings with a random prelude followed by a long repeating “1 open then 1 close” pattern. The vertical dashed line marks the maximum training length. Our model preserves strong stack-tracking performance even on long OOD sequences.}}
% %     \label{fig:dyck-accuracy}
% % \end{figure}

% % \begin{figure*}[tb]
% %     \centering
% %     \begin{subfigure}[b]{0.45\textwidth}
% %         \includegraphics[width=\textwidth]{figures/dyck/energy.pdf}
% %         \caption{Energy}
% %         \label{fig:dyck-energy}
% %     \end{subfigure}
% %     \hfill
% %     \begin{subfigure}[b]{0.26\textwidth}
% %         \includegraphics[width=\textwidth]{figures/dyck/pca_1st.pdf}
% %         \caption{Layer1 state transition}
% %         \label{fig:dyck-pca-1st}
% %     \end{subfigure}
% %     \hfill
% %     \begin{subfigure}[b]{0.26\textwidth}
% %         \includegraphics[width=\textwidth]{figures/dyck/pca_2nd.pdf}
% %         \caption{Layer2 state transition}
% %         \label{fig:dyck-pca-2nd}
% %     \end{subfigure}
% %     \caption{\rev{Comparison of Dyck dynamics on $5$-regular runs. (a) Energy traces for the ``layer1'' and ``layer2'' modules. (b) PCA of the layer1 latents at the last fast step shows a star structure where the end points correspond to the open brackets, where the color indicates the bracket type at that point. (c) PCA of the layer2 latents remains organized by stack depth (different colors for the bracket depth) and open/close state ($\circ$ for open, $\times$ for close), indicating coherent, length-general computation.}}
% %     \label{fig:results-dyck}
% % \end{figure*}

% \subsection{Reinforcement Learning}\label{sec:rl}


% % \small
% \begin{figure*}[!b]
%   \centering
%   % --- このfigure内だけ詰める ---
%   \captionsetup{font=footnotesize,skip=2pt} % 図キャプション上の空き
%   \captionsetup[sub]{font=footnotesize,skip=1pt} % subcaption上の空き
%   \setlength{\tabcolsep}{3pt} % 列間（左右の間）
%   \renewcommand{\arraystretch}{0} % 行のデフォ伸びを抑える

%   \begin{tabular}{@{}cc@{}}
%     \subcaptionbox{LavaCrossing\label{fig:lava}}{%
%       \includegraphics[width=.4\textwidth,trim=8 6 8 6,clip]{figures/rl/lava-retry-4env-bars.pdf}} &
%     \subcaptionbox{DoorKey\label{fig:doorkey}}{%
%       \includegraphics[width=.4\textwidth,trim=8 6 8 6,clip]{figures/rl/doorkey-retry-4env-bars.pdf}} \\
%     \subcaptionbox{MultiRoom\label{fig:multiroom}}{%
%       \includegraphics[width=.4\textwidth,trim=8 6 8 6,clip]{figures/rl/multiroom-retry-4env-bars.pdf}} &
%     \subcaptionbox{All tasks\label{fig:alltask}}{%
%       \includegraphics[width=.4\textwidth,trim=8 6 8 6,clip]{figures/rl/alltasks-ID_OOD-avg-bars.pdf}}
%   \end{tabular}
%   \vspace{2mm}
%   \caption{Success rates on MiniGrid tasks, averaged over 5 random seeds. Error bars denote the standard deviation across seeds. Our model(\method) consistently matches or outperforms strong sequence-model baselines and achieves superior average performance across all tasks.}
%   \label{fig:results-minigrid}
% \end{figure*}

% % \begin{figure*}[t]
% %     \centering
% %     \captionsetup[subfigure]{labelformat=empty}
% %     \captionsetup[subfigure]{labelsep=none}

% %     % 左ブロック（2枚をグループ化、合計0.48）
% %     \begin{subfigure}[b]{0.48\textwidth}
% %         \centering
% %         \begin{subfigure}[b]{0.49\linewidth}
% %             \includegraphics[width=\linewidth]{figures/rl/doorkey5x5.png}
% %             \caption{DoorKey-5x5~(ID)}
% %             \label{fig:doorkey5x5}
% %         \end{subfigure}\hfill
% %         \begin{subfigure}[b]{0.49\linewidth}
% %             \includegraphics[width=\linewidth]{figures/rl/doorkey16x16.png}
% %             \caption{DoorKey\nobreakdash-16x16~(OOD)}
% %             \label{fig:doorkey_ood}
% %         \end{subfigure}
% %         % \caption{DoorKey environments} % グループにだけキャプション付けたい場合
% %     \end{subfigure}\hfill%
% %     % 右ブロック（各0.24）
% %     \begin{minipage}[b]{0.01\textwidth}
% %       \centering
% %       \begin{tikzpicture}
% %         \draw[dashed] (0,-2.0) -- (0,2.0);
% %       \end{tikzpicture}
% %     \end{minipage}\hfill%
% %     \begin{subfigure}[b]{0.24\textwidth}
% %       \includegraphics[width=\linewidth]{figures/rl/multiroomN6.png}
% %       \caption{MultiRoom(OOD)}
% %     \end{subfigure}\hfill%
% %     \begin{subfigure}[b]{0.24\textwidth}
% %       \includegraphics[width=\linewidth]{figures/rl/lavacrossingS11N5.png}
% %       \caption{LavaCrossing(OOD)}
% %     \end{subfigure}
% %     \caption{MiniGrid tasks. 
% %     The two left panels show the increasing difficulty from ID to OOD in DoorKey. MultiRoom and LavaCrossing likewise require long-horizon memory and reasoning.}
% %     \label{fig:minigrid-description}
% % \end{figure*}



% % \begin{figure*}[h]
% %     \centering
% %     \captionsetup[subfigure]{labelformat=empty}
% %     \captionsetup[subfigure]{labelsep=none}
% %     \begin{subfigure}[b]{0.24\textwidth}
% %         \includegraphics[width=\textwidth]{figures/rl/doorkey5x5.png}
% %         \caption{DoorKey-5x5~(ID)}
% %         \label{fig:doorkey5x5}
% %     \end{subfigure}
% %     \begin{subfigure}[b]{0.24\textwidth}
% %         \includegraphics[width=\textwidth]{figures/rl/doorkey6x6.png}
% %         \caption{DoorKey-6x6~(OOD)}
% %         \label{fig:doorkey}
% %     \end{subfigure}
% %     \begin{subfigure}[b]{0.24\textwidth}
% %         \includegraphics[width=\textwidth]{figures/rl/doorkey8x8.png}
% %         \caption{DoorKey-8x8~(OOD)}
% %         \label{fig:multiroom}
% %     \end{subfigure}
% %     \begin{subfigure}[b]{0.24\textwidth}
% %         \includegraphics[width=\textwidth]{figures/rl/doorkey16x16.png}
% %         \caption{DoorKey\nobreakdash-16x16~(OOD)}
% %         \label{fig:alltask}
% %     \end{subfigure}
% %     \caption{Examples of the partially observable MiniGrid environments used in our experiments. 
% %     These tasks, such as DoorKey of increasing sizes, require long-horizon memory and reasoning to solve. 
% %     Here,~\mbox{(ID)} denotes in-distribution and~\mbox{(OOD)} denotes out-of-distribution.} 
% %     \label{fig:minigrid-description}
% % \end{figure*}



% % \begin{figure}[t]
% %     \centering
% %     \begin{minipage}{0.52\linewidth}
% %         \centering
% %         \includegraphics[width=\linewidth]{figures/rl/energy_doorkey.pdf}
% %         \caption{\rev{Energy landscape in DoorKey. The red crosses indicate that the agent is adjacent to a wall at that step.}}
% %         \label{fig:doorkey_energy}
% %     \end{minipage}
% %     \hfill
% %     \begin{minipage}{0.45\linewidth}
% %         \centering
% %         \includegraphics[width=\linewidth]{figures/rl/visualize_doorkey.png}
% %         \caption{\rev{Latent state transitions of our model in DoorKey -$16 \times 16$(OOD) }}
% %         \label{fig:doorkey_pca}
% %     \end{minipage}
% % \end{figure}
% % \begin{figure}[t]
% %     \centering
% %     \begin{minipage}{0.52\linewidth}
% %         \centering
% %         \includegraphics[width=\linewidth]{figures/rl/energy_doorkey.pdf}
% %         \subcaption{\rev{Energy traces  (Eq.\ref{eq:Kenergy})  of the trajectories along a given episode. The red cross marks the timings at which the agent's relative view changes beyond a certain threshold. }}
% %         \label{fig:doorkey_energy}
% %     \end{minipage}
% %     \hfill
% %     \begin{minipage}{0.45\linewidth}
% %         \centering
% %         \includegraphics[width=\linewidth]{figures/rl/visualize_doorkey.png}
% %         \subcaption{\rev{Latent state trajectories of 30 episodes, visualized by PCA.}}
% %         \label{fig:doorkey_pca}
% %     \end{minipage}
% %     \caption{\rev{Energy and latent state trajectories in the DoorKey-16x16 (OOD) environment.}}
% %     \label{fig:doorkey_overall}
% % \end{figure}

% % \begin{figure}[t]
% %     \centering
% %     % [t] オプションで画像の上端を揃える
% %     \begin{minipage}[t]{0.52\linewidth}
% %         \centering
% %         \includegraphics[width=\linewidth]{figures/rl/energy_doorkey.pdf}
% %         \subcaption{\rev{Energy traces (Eq.\ref{eq:Kenergy}) along an episode. The red cross marks agent view changes.}}
% %         \label{fig:doorkey_energy}
% %     \end{minipage}
% %     \hfill
% %     \begin{minipage}[t]{0.45\linewidth}
% %         \centering
% %         \includegraphics[width=\linewidth]{figures/rl/visualize_doorkey.png}
% %         \subcaption{\rev{Latent state trajectories of 30 episodes, visualized by PCA.}}
% %         \label{fig:doorkey_pca}
% %     \end{minipage}
% %     \caption{\rev{Energy and latent state trajectories in the DoorKey-16x16 (OOD) environment.}}
% %     \label{fig:doorkey_overall}
% % \end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.85\linewidth]{figures/rl/energy_doorkey.pdf}
%     \caption{
%      Energy traces (See \ref{sec:choice}) along an episode in the DoorKey-16x16 (OOD) environment. \textbf{Top:} Event history along the trajectory. See the legend of Figure~\ref{fig:doorkey_pca} for event markings.  The red cross marks the changes in agent's view. \textbf{Bottom:} Energy trajectories.  }
%     \label{fig:doorkey_energy}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.75\linewidth]{figures/rl/visualize_doorkey.png}
%     \caption{
%     Latent state trajectories of 30 episodes for DoorKey-16x16 (OOD) environment, visualized by PCA.
%     Observe that important events are forming trajectory-independent clusters.}
%     \label{fig:doorkey_pca}
% \end{figure}

% We next evaluate our model on challenging partially observable reinforcement learning tasks from the MiniGrid environment \citep{10.5555/3666122.3669331}.
% We consider three MiniGrid tasks: DoorKey, MultiRoom, and LavaCrossing (see Figure~\ref{fig:minigrid-description}). 
% In these navigation tasks, DoorKey requires the agent to pick up a key, open a door, and then reach the goal in this order. 
% MultiRoom requires the agent to open multiple doors sequentially to reach the goal. 
% LavaCrossing requires the agent to reach the goal while avoiding the lava. 
% In all tasks, the reward is provided only at the end of a successful episode (i.e., sparse rewards).  

% Most importantly, because these tasks do not provide a ground-truth supervisory sequence of actions, it is more difficult for the model to retrospectively infer which information in the episode is worth incorporating into its reasoning and consolidating into intermediate conclusions.  

% At each slow step, the agent receives an egocentric $7\times7$ observation with object/color/door-state channels.
% The agent then selects an action from the set $a_s \in \{\texttt{left}, \allowbreak \texttt{right}, \allowbreak \texttt{forward}, \allowbreak \texttt{toggle}, \allowbreak \texttt{pickup}, \allowbreak \texttt{drop}, \allowbreak \texttt{done}\}$.

% \paragraph{Setup}
% We designed our evaluation protocol to test the model’s generalization capabilities in a zero-shot transfer setting. 
% The agent is trained exclusively on the simplest ID configuration and is subsequently evaluated, without any further training, on more complex and previously unseen OOD environments, which are typically larger than the ID environments (see Table~\ref{tab:env-id-ood} in the Appendix for details). 
% We compare our model against a few competitive sequence-modeling baselines, including LSTM, Mamba-2, and Transformer-XL. 
% Results are averaged over five random seeds, and we report the mean and standard deviation.

% All models are trained end-to-end using Proximal Policy Optimization (PPO; \citet{schulman2017ppo}).  
% For our model, the agent’s encoder (sensory module) first processes the input observations through a series of convolutional layers, followed by our recurrent core (Eq.~\ref{eq:FastSlow}).
% Please see Appendix~\ref{app:rl-details} for more details.



% \paragraph{Results}
% Figure~\ref{fig:results-minigrid} shows the success rates across all MiniGrid tasks. Our model performs comparably to or better than the baselines across all tested environments. This suggests that the recurrent mechanism of \textit{thinking while listening} is effective in these complex sequential decision-making problems as well.
% Also, we again observe a clear emergent structure in the latent space of our learned model. 
% We find that fluctuations in the energy value reflect the agent's level of ``frustration'', for example, when the agent's vision changes beyond a certain threshold (Figure~\ref{fig:doorkey_energy}). 
% Figure~\ref{fig:doorkey_pca} shows PCA-projected latent state transitions for DoorKey; irrespective of the trajectories, the model organizes its representations around key-events such as the ``key pickup'', ``door opening'', and ``goal discovery.'' 


% % Figure~\ref{fig:training-curve-doorkey}



% % \textbf{Designing \texorpdfstring{$J_t(X(t), C(s(t)))$}{J_t(X(t), C(t))} with External Memory}

% % Let the fast-time index be $t=0,1,2,\dots$ and the slow index be $s(t)=\lfloor t/T\rfloor$.
% % Aggregate past information into an external memory $m_t$ and update it causally:
% % \begin{align}
% % r_t &= \rho\!\bigl(X_t,\,C(s(t))\bigr), \\
% % m_{t+1} &= F\!\bigl(m_t,\,r_t\bigr),
% % \end{align}
% % where $\rho$ reads out from the current inner-loop output, and $F$ is any causal RNN (e.g., LSTM/GRU).

% % To ensure temporal continuity, define the objective at fast time $t$ as a continuous mapping of $m_t$:
% % \begin{align}
% % J_t \;\equiv\; J\!\bigl(\,\cdot\,;\,m_t,\,C(s(t))\bigr) \;:=\; \Phi(m_t)\,,
% % \end{align}
% % and constrain $\Phi$ to be Lipschitz (e.g., via spectral normalization, $1{\times}1$ convolutions, or small-step updates). Then, for some constant $L>0$,
% % \begin{align}
% % \bigl\|J_{t+1}-J_t\bigr\| \;\le\; L\,\bigl\|m_{t+1}-m_t\bigr\|\,,
% % \end{align}
% % so $J_t$ varies smoothly over time. 
% % This external-memory formulation is especially effective when the slow interval is long, as $m_t$ preserves continuity across extended gaps in $s$.



% % \paragraph{Test Time Scaling}

% % Figure~\ref{fig:tts-rl} illustrates the impact of varying $s$ on the agent's success rate across the three MiniGrid tasks. For all tasks, performance monotonically improves as $s$ is increased. This demonstrates that our model can effectively leverage additional computational budget at test time to enhance its decision-making quality. This graceful scaling property is highly desirable, as it allows for a flexible trade-off between computational cost and performance, enabling the deployment of the same trained model in various scenarios with different resource constraints.

% % \paragraph{Scaling with respect to $s$}
% % One the desiderate of our model is to feature the ability to reasoning that scales with the observation time $s$.
% % We therefore measured the models' behavior when we allowed longer durations (larger values) of $s$. 
% % We observe that the accuracy of our method generally improves with increasing $s$ for all environments (Figure~\ref{fig:tts-rl}).
% % While it is true that, for these experiments the accuracy itself shall scale with longer lenght of the episode length, our method improves faster and saturates at higher accuracy level than the competitors.  
% % \maso{For the DoorKey environment, however, LSTM surpasses our method beyond certain episode length because ...?} 


% % We posit that this is because the task in the DoorKey environment is bottlenecked by simple key discovery: in this setting, increasing $s$ merely lengthens the agent's dwell time spent in near-random wandering, passively raising the probability of encountering the key. Conversely, success in LavaCrossing and MultiRoom is predicated on goal-directed long-range dependencies, a context where such random exploration is entirely ineffective. This explains the limited performance gains of the standard LSTM baseline in these environments. In sharp contrast, our method with auxiliary memory is specifically designed to leverage these extra inner-loop iterations, enabling it to coherently integrate past observations and systematically refine the action plan.

% % \begin{figure*}[h]
% %     \centering
% %     \begin{subfigure}[b]{0.32\textwidth}
% %         \includegraphics[width=\textwidth]{figures/rl/test_time_scaling_doorkey.png}
% %         \caption{DoorKey}
% %         %\label{fig:tts_doorkey}
% %     \end{subfigure}
% %     \hfill
% %     \begin{subfigure}[b]{0.32\textwidth}
% %         \includegraphics[width=\textwidth]{figures/rl/test_time_scaling_lava.png}
% %         \caption{LavaCrossing}
% %         %\label{fig:doorkey}
% %     \end{subfigure}
% %     \hfill
% %     \begin{subfigure}[b]{0.32\textwidth}
% %         \includegraphics[width=\textwidth]{figures/rl/test_time_scaling_multi_room.png}
% %         \caption{MultiRoom}
% %         %\label{fig:doorkey}
% %     \end{subfigure}
% %     \caption{Effect of test-time scaling on the MiniGrid tasks, plotted against $s$, the slow process time scale.  The success rate consistently improves as the number of reasoning iterations increases at test time, highlighting the model's ability to leverage additional inference loops.}
% %     \label{fig:tts-rl}
% % \end{figure*}


==> setup.tex <==
\section{Problem Setting} \label{sec:task}

We consider the setting in which the observations arrive as a stream and the model reasons and (optionally) acts while the stream is unfolding. Unlike conventional pipelines, which first ingest a long sequence and only then iterate internally, this setting requires the model’s internal reasoning to proceed in parallel with data arrival.  

To be more specific, let $(o_1,\ldots,o_{S})$ be an ordered sequence of observations that arrives at discrete \emph{data times} $s\in\{1,\ldots,S\}$, and let us denote by $\{y_s\}_{s=1}^{S}$ the time-stamped predictions of the model, and by $\mathcal{E}\subseteq\{1,\ldots,S\}$ the set of data times at which the model chooses to return an output. \rev{At test time, $S$ may exceed the values seen during training, so that the model must generalize to longer observation streams.}
%
The settings we consider can be formalized by the following \textit{\rev{causal} constraint} on the model's response:
$$
\boxed{\text{If } s^* \in\mathcal{E},\ \ y_{s^*} \text{ must be produced using only } o_{1:s^*}.}
%\text{ and is available before } o_{s^*+1}.}
$$
\rev{This constraint captures the causal nature of streaming settings: for any $s^*$, the model can only depend on past and current observations, but not on future ones.}
We refer to this problem as \task, which includes two important subtasks as special cases. In the first case, reinforcement learning, the agent must act at every step; thus $\mathcal{E}=\{1,\ldots,S\}$ and the model returns the full sequence $\{y_1,\ldots,y_{S}\}$ (where each $y_s$ is an action).
In the second case, sequential regression/classification, the model must output exactly one label at some time $s^\star\le S$. Here $\mathcal{E}=\{s^\star\}$, and the output consists of a single element from $\{y_1,\ldots,y_{S}\}$.
% \rev{This type of task is also natural for the setting in which the context length is indefinite; that is, when it is unknown when the streaming input is to end.}

%In contrast, conventional recurrent TTS methods typically wait to read the entire sequence (or a long chunk) and only then iterate; in realtime sequential reasoning the model must start reasoning at $n=1$ and meet a deadline at every step. This distinction is especially important under partial observability (e.g., POMDPs in RL) or when decisions must be made on streaming sensory input; static puzzles like Sudoku do not impose such streaming deadlines and therefore fall outside this setting.





% %  \citep{bansal2022end}
% We also mention that our philosophy is in alignment with recent advances in biological research. According to \citep{PNAsRecurrent, Markov2014WeightedDirected, Oh2014MesoscaleConnectome}, recurrent architectures are ubiquitous in nervous systems, and quantitative data on the cortical connectome indicate that recurrent connections far outnumber feedforward connections.
% \citep{OsunaOrozco2025Recurrent} conducted data assimilation of simulations based on a human brain connectivity matrix based on large-scale recordings of neural activity and verified the hierarchical clustering structure of recurrent dynamics. 

% \citep{Honey2012SlowCorticalDynamics} analyzed electrocorticographic signals and discovered that the slowly fluctuating component of the brain is associated with the accumulation of information over a longer period, suggesting a connection between slow neuronal population dynamics and temporally extended information processing.
% \citep{Song2024HierarchicalTimescalesForebrain} reports that brain activities exist in different time scales and vary in a hierarchy in relation to sensory and memory associations.

==> shortcuts.tex <==
\newcommand{\ba}{\mathbf{a}}\newcommand{\bA}{\mathbf{A}}
\newcommand{\bb}{\mathbf{b}}\newcommand{\bB}{\mathbf{B}}
\newcommand{\bc}{\mathbf{c}}\newcommand{\bC}{\mathbf{C}}
\newcommand{\bd}{\mathbf{d}}\newcommand{\bD}{\mathbf{D}}
\newcommand{\be}{\mathbf{e}}\newcommand{\bE}{\mathbf{E}}
\newcommand{\bff}{\mathbf{f}}\newcommand{\bF}{\mathbf{F}} %
\newcommand{\bg}{\mathbf{g}}\newcommand{\bG}{\mathbf{G}}
\newcommand{\bh}{\mathbf{h}}\newcommand{\bH}{\mathbf{H}}
\newcommand{\bi}{\mathbf{i}}\newcommand{\bI}{\mathbf{I}}
\newcommand{\bj}{\mathbf{j}}\newcommand{\bJ}{\mathbf{J}}
\newcommand{\bk}{\mathbf{k}}\newcommand{\bK}{\mathbf{K}}
\newcommand{\bl}{\mathbf{l}}\newcommand{\bL}{\mathbf{L}}
\newcommand{\bmm}{\mathbf{m}}\newcommand{\bM}{\mathbf{M}}
\newcommand{\bn}{\mathbf{n}}\newcommand{\bN}{\mathbf{N}}
\newcommand{\bo}{\mathbf{o}}\newcommand{\bO}{\mathbf{O}}
\newcommand{\bp}{\mathbf{p}}\newcommand{\bP}{\mathbf{P}}
\newcommand{\bq}{\mathbf{q}}\newcommand{\bQ}{\mathbf{Q}}
\newcommand{\br}{\mathbf{r}}\newcommand{\bR}{\mathbf{R}}
\newcommand{\bs}{\mathbf{s}}\newcommand{\bS}{\mathbf{S}}
\newcommand{\bt}{\mathbf{t}}\newcommand{\bT}{\mathbf{T}}
\newcommand{\bu}{\mathbf{u}}\newcommand{\bU}{\mathbf{U}}
\newcommand{\bv}{\mathbf{v}}\newcommand{\bV}{\mathbf{V}}
\newcommand{\bw}{\mathbf{w}}\newcommand{\bW}{\mathbf{W}}
\newcommand{\bx}{\mathbf{x}}\newcommand{\bX}{\mathbf{X}}
\newcommand{\by}{\mathbf{y}}\newcommand{\bY}{\mathbf{Y}}
\newcommand{\bz}{\mathbf{z}}\newcommand{\bZ}{\mathbf{Z}}

\newcommand{\balpha}{\boldsymbol{\alpha}}\newcommand{\bAlpha}{\boldsymbol{\Alpha}}
\newcommand{\bbeta}{\boldsymbol{\beta}}\newcommand{\bBeta}{\boldsymbol{\Beta}}
\newcommand{\bgamma}{\boldsymbol{\gamma}}\newcommand{\bGamma}{\boldsymbol{\Gamma}}
\newcommand{\bdelta}{\boldsymbol{\delta}}\newcommand{\bDelta}{\boldsymbol{\Delta}}
\newcommand{\bepsilon}{\boldsymbol{\epsilon}}\newcommand{\bEpsilon}{\boldsymbol{\Epsilon}}
\newcommand{\bzeta}{\boldsymbol{\zeta}}\newcommand{\bZeta}{\boldsymbol{\Zeta}}
\newcommand{\beeta}{\boldsymbol{\eta}}\newcommand{\bEta}{\boldsymbol{\Eta}} %
\newcommand{\btheta}{\boldsymbol{\theta}}\newcommand{\bTheta}{\boldsymbol{\Theta}}
\newcommand{\biota}{\boldsymbol{\iota}}\newcommand{\bIota}{\boldsymbol{\Iota}}
\newcommand{\bkappa}{\boldsymbol{\kappa}}\newcommand{\bKappa}{\boldsymbol{\Kappa}}
\newcommand{\blambda}{\boldsymbol{\lambda}}\newcommand{\bLambda}{\boldsymbol{\Lambda}}
\newcommand{\bmu}{\boldsymbol{\mu}}\newcommand{\bMu}{\boldsymbol{\Mu}}
\newcommand{\bnu}{\boldsymbol{\nu}}\newcommand{\bNu}{\boldsymbol{\Nu}}
\newcommand{\bxi}{\boldsymbol{\xi}}\newcommand{\bXi}{\boldsymbol{\Xi}}
\newcommand{\bomikron}{\boldsymbol{\omikron}}\newcommand{\bOmikron}{\boldsymbol{\Omikron}}
\newcommand{\bpi}{\boldsymbol{\pi}}\newcommand{\bPi}{\boldsymbol{\Pi}}
\newcommand{\brho}{\boldsymbol{\rho}}\newcommand{\bRho}{\boldsymbol{\Rho}}
\newcommand{\bsigma}{\boldsymbol{\sigma}}\newcommand{\bSigma}{\boldsymbol{\Sigma}}
\newcommand{\btau}{\boldsymbol{\tau}}\newcommand{\bTau}{\boldsymbol{\Tau}}
\newcommand{\bypsilon}{\boldsymbol{\ypsilon}}\newcommand{\bYpsilon}{\boldsymbol{\Ypsilon}}
\newcommand{\bphi}{\boldsymbol{\phi}}\newcommand{\bPhi}{\boldsymbol{\Phi}}
\newcommand{\bchi}{\boldsymbol{\chi}}\newcommand{\bChi}{\boldsymbol{\Chi}}
\newcommand{\bpsi}{\boldsymbol{\psi}}\newcommand{\bPsi}{\boldsymbol{\Psi}}
\newcommand{\bomega}{\boldsymbol{\omega}}\newcommand{\bOmega}{\boldsymbol{\Omega}}

\newcommand{\nA}{\mathbb{A}}
\newcommand{\nB}{\mathbb{B}}
\newcommand{\nC}{\mathbb{C}}
\newcommand{\nD}{\mathbb{D}}
\newcommand{\nE}{\mathbb{E}}
\newcommand{\nF}{\mathbb{F}}
\newcommand{\nG}{\mathbb{G}}
\newcommand{\nH}{\mathbb{H}}
\newcommand{\nI}{\mathbb{I}}
\newcommand{\nJ}{\mathbb{J}}
\newcommand{\nK}{\mathbb{K}}
\newcommand{\nL}{\mathbb{L}}
\newcommand{\nM}{\mathbb{M}}
\newcommand{\nN}{\mathbb{N}}
\newcommand{\nO}{\mathbb{O}}
\newcommand{\nP}{\mathbb{P}}
\newcommand{\nQ}{\mathbb{Q}}
\newcommand{\nR}{\mathbb{R}}
\newcommand{\nS}{\mathbb{S}}
\newcommand{\nT}{\mathbb{T}}
\newcommand{\nU}{\mathbb{U}}
\newcommand{\nV}{\mathbb{V}}
\newcommand{\nW}{\mathbb{W}}
\newcommand{\nX}{\mathbb{X}}
\newcommand{\nY}{\mathbb{Y}}
\newcommand{\nZ}{\mathbb{Z}}

\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

\newcommand{\shortsecref}[1]{Sec.~\ref{#1}}

\newcommand{\eqnref}[1]{Eq.~\eqref{#1}}
\newcommand{\tabref}[1]{Table~\ref{#1}}


\def\mc{\mathcal}
\def\mb{\mathbf}

\newcommand{\T}{^{\raisemath{-1pt}{\mathsf{T}}}}

\newcommand{\Perp}{\perp\!\!\! \perp}


\newcommand*\rot{\rotatebox{90}}

\newcommand{\boldparagraph}[1]{\vspace{0.0cm}\noindent{\bf #1:} }
\newcommand{\boldparagraphnocolon}[1]{\vspace{0.0cm}\noindent{\bf #1}}

\definecolor{darkgreen}{rgb}{0,0.7,0}
\definecolor{darkblue}{RGB}{31,119,180}
\definecolor{darkred}{RGB}{214,39,40}
\definecolor{mediumgray}{rgb}{0.5,0.5,0.5}
\definecolor{mediumteal}{rgb}{0,0.5,0.5}

\definecolor{ellisred}{rgb}{0.87,0.44,0.38} %
\definecolor{ellisgreen}{rgb}{0.69,0.90,0.52} %
\definecolor{elliscyan}{rgb}{0.29,0.77,0.74} %
\definecolor{ellisorange}{rgb}{0.89,0.55,0.28} %
\definecolor{ellisblue}{rgb}{0.41,0.61,0.86} %

\newcommand{\ellisred}[1]{\noindent{\color{ellisred}{#1}}}
\newcommand{\ellisgreen}[1]{\noindent{\color{ellisgreen}{#1}}}
\newcommand{\elliscyan}[1]{\noindent{\color{elliscyan}{#1}}}
\newcommand{\ellisorange}[1]{\noindent{\color{ellisorange}{#1}}}
\newcommand{\ellisblue}[1]{\noindent{\color{ellisblue}{#1}}}

\newcommand{\singleitem}{\noindent \textbullet$~$}
\newcommand{\pmsd}[1]{{\color{mediumgray}{\scriptsize $\pm$ #1}}}
